6DLS: Modeling Nonplanar Frictional Surface Contacts for Grasping using 6D Limit Surfaces

Robot grasping with deformable gripper jaws results in nonplanar surface contacts if the jaws deform to the nonplanar local geometry of an object. The frictional force and torque that can be transmitted through a nonplanar surface contact are both three-dimensional, resulting in a six-dimensional frictional wrench (6DFW). Applying traditional planar contact models to such contacts leads to over-conservative results as the models do not consider the nonplanar surface geometry and only compute a three-dimensional subset of the 6DFW. To address this issue, we derive the 6DFW for nonplanar surfaces by combining concepts of differential geometry and Coulomb friction. We also propose two 6D limit surface (6DLS) models, generalized from well-known three-dimensional LS (3DLS) models, which describe the friction-motion constraints for a contact. We evaluate the 6DLS models by fitting them to the 6DFW samples obtained from six parametric surfaces and 2,932 meshed contacts from finite element method simulations of 24 rigid objects. We further present an algorithm to predict multicontact grasp success by building a grasp wrench space with the 6DLS model of each contact. To evaluate the algorithm, we collected 1,035 physical grasps of ten 3D-printed objects with a KUKA robot and a deformable parallel-jaw gripper. In our experiments, the algorithm achieves 66.8% precision, a metric inversely related to false positive predictions, and 76.9% recall, a metric inversely related to false negative predictions. The 6DLS models increase recall by up to 26.1% over 3DLS models with similar precision.

==> figs/figDBParameters.tex <==
\begin{figure}[!t]
	%\vspace{-0.7em}
	\centering	
		\subfloat[]{{\includegraphics[width=41mm,trim={0cm 0cm 0cm 0cm}, clip]{figs/sources/FEM/gen-params}  }}% 	
		\hspace{-1.5em}	
		\qquad
		\subfloat[]{{\includegraphics[width=41mm,trim={0cm 0cm 0cm 0cm}, clip]{figs/sources/FEM/gen-models}  }}% 			
	\caption{Parametric generation of the thin-walled objects for FEM simulations. (a) The geometry is controlled with an elliptic base and a spline for the wall (Figure recreated from \cite{Alt.2016.dataset}). (b) Ellipses are created at sampled heights $E_{1,\ldots,n}$ and adjacent ellipses rule smooth surfaces. The square/circles show the locations of antipodal grasps used in simulations.} %The curvature of the sections are controlled by the variables $p_{1,\ldots,7}$. 
	\label{fig:db_parameters}
\end{figure}




==> figs/figFEMAnsys.tex <==
\begin{figure}
	%\vspace{-0.7em}
	\centering	
	\subfloat[Beam-shaped jaws.]{{\includegraphics[height=36mm,trim={0cm 0.4cm 0cm 0cm}, clip]{figs/sources/FEM/Finger-Beam-meshed-proc} }}% 	
	\qquad
	\hspace{-2.2em}
	\subfloat[Simulation results.]{{\includegraphics[height=36mm,trim={2.1cm 0.5cm 3.1cm 0.5cm}, clip]{figs/sources/FEM/Finger-Beam-simulated-proc-num} }}% 	
	

	\subfloat[Elliptical fingertip.]{{\includegraphics[height=36mm,trim={0cm 0.3cm 0cm 0cm}, clip]{figs/sources/FEM/Finger-Ellipse-meshed-proc} }}% 	
	\qquad
	\hspace{-2.2em}
	\subfloat[Simulation results.]{{\includegraphics[height=36mm,trim={2.1cm 0.5cm 3.1cm 0.5cm}, clip]{figs/sources/FEM/Finger-ellipsoid-simulation-proc-num}  }}% 	


%	\subfloat[object 1.]{{\includegraphics[width=93mm,trim={1cm 8.5cm 0.5cm 7cm}, clip]{fig/FEM/fig9} }}% 	
%	\qquad
%	\hspace{-3.8em}
%	\subfloat[object 1.]{{\includegraphics[width=91mm,trim={1cm 7cm 1cm 9.5cm}, clip]{fig/FEM/fig7}  }}% 			
				
	\caption{An object is grasped with beam-shaped and ellipsoidal deformable jaws. (a) and (c) show the initial state of the meshed object and jaws, while (b) and (d) illustrate the deformed jaws and the pressure distribution of the contacts after the simulation. The contact profile is then  used to compute wrench/twist pairs and to evaluate the fitting results of the proposed 6DLS models.}
	\label{fig:FEM_sim}%
\end{figure}




==> figs/figLS4th.tex <==

\begin{figure*}
	%\vspace{-0.7em}
	\centering	
	\subfloat[ $(f_x,f_y,f_z,0,0,0)^T$.]{{\includegraphics[width=48mm,trim={0.6cm 5.8cm  0.9cm 6cm}, clip]{figs/sources/ls4/fig1} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[ $(f_x,f_y,0,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig2} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[ $(f_x,f_y,0,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig3} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[  $(f_x,f_y,0,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig4} }}% 	
	
	\subfloat[$(f_x,0,f_z,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig5} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,f_z,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig6} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,f_z,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig7} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,0,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig8} }}% 	

	\subfloat[$(f_x,0,0,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig9} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,0,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig10} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,f_z,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig11} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,f_z,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig12} }}% 	

	\subfloat[$(0,f_y,f_z,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig13} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig14} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig15} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig16} }}% 	

	\subfloat[$(0,0,f_z,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig17} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,f_z,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig18} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,f_z,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig19} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,0,\tau_x,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig20} }}% 	
	\caption{3D cross-sections of a quartic 6D limit surface fit to wrench and twist pairs.}
	\label{fig:LS4th}%
\end{figure*}




==> figs/figLS4thbc.tex <==

\begin{figure*}
	%\vspace{-0.7em}
	\centering	
	\subfloat[ $(f_x,f_y,f_z,0,0,0)^T$.]{{\includegraphics[width=48mm,trim={0.6cm 5.8cm  0.9cm 6cm}, clip]{fig/ls4/fig1} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[ $(f_x,f_y,0,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig2} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[ $(f_x,f_y,0,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig3} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[  $(f_x,f_y,0,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig4} }}% 	
	
	\subfloat[$(f_x,0,f_z,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig5} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,f_z,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig6} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,f_z,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig7} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,0,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig8} }}% 	

	\subfloat[$(f_x,0,0,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig9} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,0,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig10} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,f_z,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig11} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,f_z,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig12} }}% 	

	\subfloat[$(0,f_y,f_z,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig13} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig14} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig15} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig16} }}% 	

	\subfloat[$(0,0,f_z,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig17} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,f_z,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig18} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,f_z,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig19} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,0,\tau_x,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{fig/ls4/fig20} }}% 	
	\caption{Cross-sections of a fitted six-dimensional quartic polynomial limit surface model.}
	\label{fig:LS4th}%
\end{figure*}




==> figs/figLSEllip.tex <==

\begin{figure*}
	%\vspace{-0.7em}
	\centering	
	\subfloat[ $(f_x,f_y,f_z,0,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  0.9cm 6cm}, clip]{figs/sources/ls2/fig1} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[ $(f_x,f_y,0,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig2} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[ $(f_x,f_y,0,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig3} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[  $(f_x,f_y,0,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig4} }}% 	
	
	\subfloat[$(f_x,0,f_z,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig5} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,f_z,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig6} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,f_z,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig7} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,0,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig8} }}% 	
	
	\subfloat[$(f_x,0,0,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig9} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,0,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig10} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,f_z,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig11} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,f_z,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig12} }}% 	
	
	\subfloat[$(0,f_y,f_z,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig13} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig14} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig15} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.3cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig16} }}% 	
	
	\subfloat[$(0,0,f_z,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.4cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig17} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,f_z,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig18} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,f_z,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig19} }}% 	s
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,0,\tau_x,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.6cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig20} }}% 	
	\caption{3D cross-sections of an ellipsoidal 6D limit surface fit to wrench and twist pairs.}
	\label{fig:LS2nd}%
\end{figure*}




==> figs/figLSEllipbc.tex <==

\begin{figure*}
	%\vspace{-0.7em}
	\centering	
	\subfloat[ $(f_x,f_y,f_z,0,0,0)^T$.]{{\includegraphics[width=48mm,trim={0.6cm 5.8cm  0.9cm 6cm}, clip]{figs/sources/ls2/fig1} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[ $(f_x,f_y,0,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig2} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[ $(f_x,f_y,0,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig3} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[  $(f_x,f_y,0,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig4} }}% 	
	
	\subfloat[$(f_x,0,f_z,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig5} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,f_z,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig6} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,f_z,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig7} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,0,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig8} }}% 	
	
	\subfloat[$(f_x,0,0,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig9} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(f_x,0,0,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig10} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,f_z,\tau_x,0,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig11} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,f_z,0,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig12} }}% 	
	
	\subfloat[$(0,f_y,f_z,0,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig13} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig14} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig15} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,f_y,0,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig16} }}% 	
	
	\subfloat[$(0,0,f_z,\tau_x,\tau_y,0)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig17} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,f_z,\tau_x,0,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig18} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,f_z,0,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls2/fig19} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[$(0,0,0,\tau_x,\tau_y,\tau_z)^T$.]{{\includegraphics[width=47mm,trim={0.8cm 5.8cm  1.5cm 7.6cm}, clip]{figs/sources/ls4/fig20} }}% 	
	\caption{Cross-sections of a fitted six-dimensional ellipsoidal limit surface model.}
	\label{fig:LS2nd}%
\end{figure*}




==> figs/figObjModels.tex <==
\begin{figure*}
	%\vspace{-0.7em}
	\centering	
	\subfloat[]{{\includegraphics[width=16mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig1} }}% 	
	\qquad
	\hspace{-3.3em}
	\subfloat[]{{\includegraphics[width=16mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig2} }}% 	
	\qquad
	\hspace{-3.3em}
	\subfloat[]{{\includegraphics[width=16mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig3} }}% 	
	\qquad
	\hspace{-3.3em}
	\subfloat[]{{\includegraphics[width=16mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig4} }}% 	
	\qquad
	\hspace{-3.3em}
	\subfloat[]{{\includegraphics[width=16mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig5} }}% 	
	\qquad
	\hspace{-3.3em}
	\subfloat[]{{\includegraphics[width=16mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig6} }}% 
	\qquad
	\hspace{-3.4em}	
	\subfloat[]{{\includegraphics[width=16mm,trim={7.5cm 8.3cm 5cm 7.9cm},clip]{figs/sources/models/fig7} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=16mm,trim={4cm 8.3cm 3cm 7.9cm},clip]{figs/sources/models/fig8} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={4cm 8.5cm 3cm 7.9cm}, clip]{figs/sources/models/fig9} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={7.2cm 9cm 5cm 7.6cm}, clip]{figs/sources/models/fig10} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={6.8cm 8.8cm 5cm 7.6cm}, clip]{figs/sources/models/fig11} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={7cm 8.8cm 5cm 7.6cm},clip]{figs/sources/models/fig12} }}% 		
		
	
	
	

	\subfloat[]{{\includegraphics[width=15.3mm,trim={7.5cm 9cm 5cm 7.9cm},clip]{figs/sources/models/fig13} }}% 
	\qquad	
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={7.5cm 8.2cm 5cm 7.9cm},clip]{figs/sources/models/fig14} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={7.2cm 8.2cm 5cm 7.9cm},clip]{figs/sources/models/fig15} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={6.5cm 8.2cm 5cm 7.6cm}, clip]{figs/sources/models/fig16} }}% 	
	\qquad
	\hspace{-2em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={6cm 8.5cm 3cm 7.5cm}, clip]{figs/sources/models/fig17} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={5.8cm 8.5cm 3cm 7.5cm},clip]{figs/sources/models/fig18} }}% 		
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={6cm 8.2cm 5cm 7cm},clip]{figs/sources/models/fig19} }}% 	
	\hspace{-1em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={5.2cm 8.2cm 4cm 7.6cm},clip]{figs/sources/models/fig20} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={5.8cm 8.2cm 4.8cm 7.6cm},clip]{figs/sources/models/fig21} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={5.5cm 8.2cm 4cm 7.6cm}, clip]{figs/sources/models/fig22} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={5.5cm 8.5cm 1.5cm 7.5cm}, clip]{figs/sources/models/fig23} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[]{{\includegraphics[width=15.3mm,trim={5cm 8.5cm 3cm 7.5cm},clip]{figs/sources/models/fig24} }}% 	
	
	\caption{24 Non-uniform rational B-Spline (NURBS)-based objects used for FEM simulations to create a large variety of contact profiles. Objects in (q)-(x) are asymmetric.}
	\label{fig:fem_objects}%
\end{figure*}





%\begin{figure*}
%	%\vspace{-0.7em}
%	\centering	
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig1} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig2} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig3} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig4} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig5} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig6} }}% 	
%	
%	\vspace{-0.5em}
%	\subfloat[object 7.]{{\includegraphics[width=29mm,trim={7.5cm 8.3cm 5cm 7.9cm},clip]{fig/models/fig7} }}% 	
%	\hspace{-2em}
%	\subfloat[object 8.]{{\includegraphics[width=29mm,trim={4cm 8.3cm 3cm 7.9cm},clip]{fig/models/fig8} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 9]{{\includegraphics[width=29mm,trim={4cm 8.5cm 3cm 7.9cm}, clip]{fig/models/fig9} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={7.2cm 9cm 5cm 7.6cm}, clip]{fig/models/fig10} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={6.8cm 8.8cm 5cm 7.6cm}, clip]{fig/models/fig11} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={7cm 8.8cm 5cm 7.6cm},clip]{fig/models/fig12} }}% 	
%	
%	\vspace{-0.5em}
%	
%	\subfloat[object 7.]{{\includegraphics[width=29mm,trim={7.5cm 9cm 5cm 7.9cm},clip]{fig/models/fig13} }}% 	
%	\hspace{-2em}
%	\subfloat[object 8.]{{\includegraphics[width=29mm,trim={7.5cm 8.2cm 5cm 7.9cm},clip]{fig/models/fig14} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 9]{{\includegraphics[width=29mm,trim={7.2cm 8.2cm 5cm 7.9cm},clip]{fig/models/fig15} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={6.5cm 8.2cm 5cm 7.6cm}, clip]{fig/models/fig16} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={6cm 8.5cm 3cm 7.5cm}, clip]{fig/models/fig17} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={5.8cm 8.5cm 3cm 7.5cm},clip]{fig/models/fig18} }}% 		
%	
%	
%	\vspace{-0.5em}
%	\subfloat[object 7.]{{\includegraphics[width=29mm,trim={6cm 8.2cm 5cm 7cm},clip]{fig/models/fig19} }}% 	
%	\hspace{-1em}
%	\subfloat[object 8.]{{\includegraphics[width=29mm,trim={5.2cm 8.2cm 4cm 7.6cm},clip]{fig/models/fig20} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 9]{{\includegraphics[width=29mm,trim={5.8cm 8.2cm 4.8cm 7.6cm},clip]{fig/models/fig21} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={5.5cm 8.2cm 4cm 7.6cm}, clip]{fig/models/fig22} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={5.5cm 8.5cm 1.5cm 7.5cm}, clip]{fig/models/fig23} }}% 	
%	\qquad
%	\hspace{-4.5em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={5cm 8.5cm 3cm 7.5cm},clip]{fig/models/fig24} }}% 	
%	
%	\caption{Fitted Limit surface with 4th order poly model.}
%	\label{fig:oob_error}%
%\end{figure*}
%
%


==> figs/figObjModels3lines.tex <==
\begin{figure*}
	%\vspace{-0.7em}
	\centering	
	\subfloat[object 1.]{{\includegraphics[width=24mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig1} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[object 2.]{{\includegraphics[width=24mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig2} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[object 3.]{{\includegraphics[width=24mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig3} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[object 4.]{{\includegraphics[width=24mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig4} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[object 5.]{{\includegraphics[width=24mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig5} }}% 	
	\qquad
	\hspace{-3.5em}
	\subfloat[object 6.]{{\includegraphics[width=24mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{figs/sources/models/fig6} }}% 
	\hspace{-3.5em}	
	\qquad
	\subfloat[object 7.]{{\includegraphics[width=24mm,trim={7.5cm 8.3cm 5cm 7.9cm},clip]{figs/sources/models/fig7} }}% 	
	\hspace{-2em}
	\subfloat[object 8.]{{\includegraphics[width=24mm,trim={4cm 8.3cm 3cm 7.9cm},clip]{figs/sources/models/fig8} }}% 	
	
	
	

	\subfloat[object 9.]{{\includegraphics[width=23mm,trim={4cm 8.5cm 3cm 7.9cm}, clip]{figs/sources/models/fig9} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 10.]{{\includegraphics[width=23mm,trim={7.2cm 9cm 5cm 7.6cm}, clip]{figs/sources/models/fig10} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 11.]{{\includegraphics[width=23mm,trim={6.8cm 8.8cm 5cm 7.6cm}, clip]{figs/sources/models/fig11} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 12.]{{\includegraphics[width=23mm,trim={7cm 8.8cm 5cm 7.6cm},clip]{figs/sources/models/fig12} }}% 		
	\qquad	
	\hspace{-3em}
	\subfloat[object 13.]{{\includegraphics[width=23mm,trim={7.5cm 9cm 5cm 7.9cm},clip]{figs/sources/models/fig13} }}% 	
	\hspace{-2em}
	\subfloat[object 14.]{{\includegraphics[width=23mm,trim={7.5cm 8.2cm 5cm 7.9cm},clip]{figs/sources/models/fig14} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 15.]{{\includegraphics[width=23mm,trim={7.2cm 8.2cm 5cm 7.9cm},clip]{figs/sources/models/fig15} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 16.]{{\includegraphics[width=23mm,trim={6.5cm 8.2cm 5cm 7.6cm}, clip]{figs/sources/models/fig16} }}% 	
	
	
	

	\subfloat[object 17.]{{\includegraphics[width=23mm,trim={6cm 8.5cm 3cm 7.5cm}, clip]{figs/sources/models/fig17} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 18.]{{\includegraphics[width=23mm,trim={5.8cm 8.5cm 3cm 7.5cm},clip]{figs/sources/models/fig18} }}% 		
	\qquad
	\hspace{-3em}
	\subfloat[object 19.]{{\includegraphics[width=23mm,trim={6cm 8.2cm 5cm 7cm},clip]{figs/sources/models/fig19} }}% 	
	\hspace{-1em}
	\subfloat[object 20.]{{\includegraphics[width=23mm,trim={5.2cm 8.2cm 4cm 7.6cm},clip]{figs/sources/models/fig20} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 21.]{{\includegraphics[width=23mm,trim={5.8cm 8.2cm 4.8cm 7.6cm},clip]{figs/sources/models/fig21} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 22.]{{\includegraphics[width=23mm,trim={5.5cm 8.2cm 4cm 7.6cm}, clip]{figs/sources/models/fig22} }}% 	
	\qquad
	\hspace{-3em}
	\subfloat[object 23.]{{\includegraphics[width=23mm,trim={5.5cm 8.5cm 1.5cm 7.5cm}, clip]{figs/sources/models/fig23} }}% 	
	\qquad
	\hspace{-4em}
	\subfloat[object 24.]{{\includegraphics[width=23mm,trim={5cm 8.5cm 3cm 7.5cm},clip]{figs/sources/models/fig24} }}% 	
	
	\caption{24 Non-uniform rational B-Spline (NURBS)-based objects used for simulations. Objects 17-24 are asymmetric.}
	\label{fig:fem_objects}%
\end{figure*}





%\begin{figure*}
%	%\vspace{-0.7em}
%	\centering	
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig1} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig2} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig3} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig4} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig5} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1.]{{\includegraphics[width=29mm,trim={8.1cm 8cm 5.1cm 7.9cm}, clip]{fig/models/fig6} }}% 	
%	
%	\vspace{-0.5em}
%	\subfloat[object 7.]{{\includegraphics[width=29mm,trim={7.5cm 8.3cm 5cm 7.9cm},clip]{fig/models/fig7} }}% 	
%	\hspace{-2em}
%	\subfloat[object 8.]{{\includegraphics[width=29mm,trim={4cm 8.3cm 3cm 7.9cm},clip]{fig/models/fig8} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 9]{{\includegraphics[width=29mm,trim={4cm 8.5cm 3cm 7.9cm}, clip]{fig/models/fig9} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={7.2cm 9cm 5cm 7.6cm}, clip]{fig/models/fig10} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={6.8cm 8.8cm 5cm 7.6cm}, clip]{fig/models/fig11} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={7cm 8.8cm 5cm 7.6cm},clip]{fig/models/fig12} }}% 	
%	
%	\vspace{-0.5em}
%	
%	\subfloat[object 7.]{{\includegraphics[width=29mm,trim={7.5cm 9cm 5cm 7.9cm},clip]{fig/models/fig13} }}% 	
%	\hspace{-2em}
%	\subfloat[object 8.]{{\includegraphics[width=29mm,trim={7.5cm 8.2cm 5cm 7.9cm},clip]{fig/models/fig14} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 9]{{\includegraphics[width=29mm,trim={7.2cm 8.2cm 5cm 7.9cm},clip]{fig/models/fig15} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={6.5cm 8.2cm 5cm 7.6cm}, clip]{fig/models/fig16} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={6cm 8.5cm 3cm 7.5cm}, clip]{fig/models/fig17} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={5.8cm 8.5cm 3cm 7.5cm},clip]{fig/models/fig18} }}% 		
%	
%	
%	\vspace{-0.5em}
%	\subfloat[object 7.]{{\includegraphics[width=29mm,trim={6cm 8.2cm 5cm 7cm},clip]{fig/models/fig19} }}% 	
%	\hspace{-1em}
%	\subfloat[object 8.]{{\includegraphics[width=29mm,trim={5.2cm 8.2cm 4cm 7.6cm},clip]{fig/models/fig20} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 9]{{\includegraphics[width=29mm,trim={5.8cm 8.2cm 4.8cm 7.6cm},clip]{fig/models/fig21} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={5.5cm 8.2cm 4cm 7.6cm}, clip]{fig/models/fig22} }}% 	
%	\qquad
%	\hspace{-3em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={5.5cm 8.5cm 1.5cm 7.5cm}, clip]{fig/models/fig23} }}% 	
%	\qquad
%	\hspace{-4.5em}
%	\subfloat[object 1]{{\includegraphics[width=29mm,trim={5cm 8.5cm 3cm 7.5cm},clip]{fig/models/fig24} }}% 	
%	
%	\caption{Fitted Limit surface with 4th order poly model.}
%	\label{fig:oob_error}%
%\end{figure*}
%
%


==> sections/18-sup-simulation.tex <==


\input{figs/figDBParameters}



\subsection{FEM simulations}
\label{sec:sub-FEM}


We describe the object models with non-uniform rational B-Splines (NURBS) and use a commercial software ANSYS \cite{ansys} for the simulations, which provides a high-quality meshing tool and accurate simulation results.
The objects are generated based on the synthetic dataset of thin-walled deformable objects from our previous work \cite{alt.2016}. 
Fig. \ref{fig:db_parameters}(a) depicts the parametric generation of the object geometry. 
An ellipse defines the base and a spline curve shape the wall, which is controlled by variables $p_{1\ldots12}$.
We then vertically sample the curve and create an ellipse at each sample, where adjacent ellipses rule the object surface, as illustrated in Fig.~\ref{fig:db_parameters}(b).
The squares and circles mark the locations of antipodal grasps with two approach directions.
By varying parameters $p_{1\ldots12}$, we efficiently generate 24 objects for simulation, as shown in Fig. \ref{fig:fem_objects}, where objects in \ref{fig:fem_objects} (q)-(x) are asymmetric. 
We simulate contacts at each grasp location with two types of gripper jaws with five normal forces in range of 2-13N and results in total 2473 contacts. 



==> sections/19-sup-physical.tex <==
%\subsection{Wrench disturbances generation}
\label{app:sub-physical}




\begin{figure}
	\centering
%	\subfloat[Bottom view of the setup with examplenary locations of weight plates.]{{\includegraphics[width=85mm,trim={0cm 0cm 0cm 0cm}, clip]{figs/sources/distSetupBlue.pdf} }}% 
	\includegraphics[width=77mm,trim={0.01cm 0cm 0.3cm 3.4cm}, clip]{figs/sources/graspHorizontalBlueWeights} % 	
	\caption{\small A horizontal grasp that generates wrench disturbances in the $f_z\tau_x\tau_y$-space in the object frame. The blue circles mark the representative locations of the weight plates.}
	\label{fig:horizontal}
\end{figure}

% \begin{figure}
% 	\centering
% 	%	\subfloat[Bottom view of the setup with examplenary locations of weight plates.]{{\includegraphics[width=85mm,trim={0cm 0cm 0cm 0cm}, clip]{figs/sources/distSetupBlue.pdf} }}% 
% 	\subfloat[Wrenches of horizontal grasps.]{{\includegraphics[width=43mm,trim={0cm 6cm 1cm 7cm}, clip]{figs/sources/wrenchDist2} }}% 	
% 	\hspace{-2.5em}
% 	\qquad
% 	\subfloat[Wrenches of vertical grasps.]{{\includegraphics[width=43mm,trim={0cm 6cm 1cm 7cm}, clip]{figs/sources/wrenchDist1} }}% 
% 	\caption{Well-distributed wrench disturbances used for the experiments.}
% 	\label{fig:disturbance-setup}
% \end{figure}



%Fig. \ref{fig:disturbance-setup}(a) shows a bottom view of the 3D printed setup to create wrench disturbances with exemplary locations of the weight plates.
%%The jaw design is adapted from the Festo Fin-Ray \  structure \cite{festo}.
%%The customized jaws use a softer plastic, so that the deformed shape better adapts to the object local geometry for more reliable grasps.
%While the setup creates 3D wrenches in the world coordinate, we are able to evaluate five dimensions of the 6DLS in the object frame by using two approach directions for the grasps, where the directions are illustrated Fig. \ref{fig:graspDirections} and the arrows mark the object frame.
%%The grasps in vertical direction evaluate the disturbances in the $f_y\tau_x\tau_z$-space and horizontal grasps evaluate disturbances in the $f_z\tau_x\tau_y$-space. 
%Fig. \ref{fig:disturbance-setup}(b) and (c) illustrate the well-scatted wrench disturbances tested in the experiments.
%


%\begin{figure}
%	\centering
%	%	\subfloat[objects.]{{\includegraphics[width=81mm,trim={16cm 10cm 12cm 20cm}, clip]{fig/objectsLight} }}% 	
%	\subfloat[Objects]{{\includegraphics[width=81mm,trim={0cm 0cm 0cm 0cm}, clip]{figs/sources/objectsLight} }}% 	
%	
%%	\subfloat[Type 1.]{{\includegraphics[width=38mm,trim={0.15cm 0cm 0cm 3cm}, clip]{figs/sources/object1} }}% 	
%%	\hspace{-1.5em}	
%%	\qquad
%%	\subfloat[Type 2.]{{\includegraphics[width=38mm,trim={0cm 0cm 0cm 3cm}, clip]{figs/sources/object2} }}% 
%%	
%	%	\qquad
%	%	\subfloat[Type 3.]{{\includegraphics[width=27mm,trim={0cm 0cm 0cm 0cm}, clip]{figs/sources/object3} }}% 	
%	\caption{Ten objects for two types of contact surfaces.}
%	\label{fig:objects}
%\end{figure}









==> sections/old/0-notation-twist.tex <==
%%% math
\newcommand{\R}{\mathbb{R}}
\def\R#1{\mathbb{R}^{#1}}

%%% screw motion
% \newcommand{\twist}{\boldsymbol{t}}
\newcommand{\twistnobold}{{\xi}}
\newcommand{\twist}{\boldsymbol{\twistnobold}}

\newcommand{\normaltwist}{\hat{\boldsymbol{\twist}}}
\newcommand{\lineISA}{l}
\newcommand{\linedir}{\boldsymbol{e}}
\newcommand{\linepoint}{\boldsymbol{q}}
\newcommand{\vel}{{\boldsymbol{v}}}
\newcommand{\vpara}{{\boldsymbol{v}}_{\parallel}}
\newcommand{\vperp}{{\boldsymbol{v}}_{\perp}}
\newcommand{\angular}{{\boldsymbol{\omega}}}
\newcommand{\normang}{{\norm{\boldsymbol{\omega}}}}

%%% friction general
\newcommand{\pressure}{p}
\newcommand{\pressureunit}{\hat{\pressure}}
\newcommand{\boldf}{\boldsymbol{f}}
\newcommand{\boldtau}{\boldsymbol{\tau}}
\newcommand{\arm}{\boldsymbol{r}}

\newcommand{\wrenchnobold}{{w}}
\newcommand{\wrench}{\boldsymbol{\wrenchnobold}}
\newcommand{\normalwrench}{\hat{\wrench}}

\newcommand{\origin}{{\boldsymbol{o}}}
\newcommand{\originx}{{{o}_x}}
\newcommand{\originy}{{{o}_y}}
\newcommand{\originz}{{{o}_z}}
%%% friction for parametric surfaces
\newcommand{\boldsigma}{\boldsymbol{\sigma}}

\newcommand{\surface}{\mathcal{S}}
\newcommand{\tangent}{T_{\surface}}

\newcommand{\velfunc}{{\boldsymbol{v}}(u,v)}
\newcommand{\vrfunc}{\hat{\boldsymbol{v}}_r(u,v)}
\newcommand{\vr}{\hat{\boldsymbol{v}}_r}

\newcommand{\normalfunc}{\boldsymbol{n}(u,v)}

% \newcommand{\vtpara}{\tilde{\boldsymbol{v}}_{t_\parallel}}
% \newcommand{\vtperp}{\tilde{\boldsymbol{v}}_{t_\perp}}
\newcommand{\scalar}{k}
\newcommand{\scalarfunc}{\scalar(u,v)}
\newcommand{\normal}{\boldsymbol{n}}
\newcommand{\boldomega}{\boldsymbol{\omega}}

%%%%% friction discrete surface
\newcommand{\centeri}{\boldsymbol{c}_{i}}
\newcommand{\normali}{\normal_{i}}
\newcommand{\vri}{\hat{\boldsymbol{v}}_{r_i}}
\newcommand{\vti}{\tilde{\boldsymbol{v}}_{i}}
\newcommand{\areai}{a_{i}}
\newcommand{\pressurei}{\pressure_{i}}

%%%%%% LS fitting
\newcommand{\predt}{\twist_\text{pred}}
\newcommand{\weight}{\beta}
\newcommand{\x}{\normalwrench}
\newcommand{\xnb}{\hat{w}}

\newcommand{\A}{\matr{A}}
\newcommand{\Ae}{\A_e}
\newcommand{\Aq}{\A_q}
% \newcommand{\fe}{f_e}
% \newcommand{\fq}{f_q}
\newcommand{\fe}{f_1}
\newcommand{\fq}{f_2}

\newcommand{\nprs}{P}
\newcommand{\W}{\mathcal{W}}
\newcommand{\twistrel}{\twist_r}
\newcommand{\twistreli}{\twist_{r_i}}



%%%%%% multi contact

\newcommand{\ASP}{\A(\surface,\pressureunit)}
% \newcommand{\ASPid}{\Afit_{\idcon}(\surface_\idcon,\pressureunit_\idcon)}

\newcommand{\F}{\mathcal{F}}


\newcommand{\boldW}{\matr{W}}
\newcommand{\wext}{\boldsymbol{w}_\text{ext}}
\newcommand{\wrenchapprc}{\tilde{\boldsymbol{w}}}
\newcommand{\contactw}{{\boldsymbol{c}}}
\newcommand{\contactwunit}{\hat{\boldsymbol{c}}}
\newcommand{\fest}{\hat{\boldsymbol{f}}}
\newcommand{\tauest}{\hat{\boldsymbol{\tau}}}
\newcommand{\fperp}{{\boldsymbol{f}_\perp}}
\newcommand{\fperpiunit}{{\hat{\boldsymbol{f}}_{\perp_i}}}

\newcommand{\error}{\epsilon}
\newcommand{\errorwrench}{{\error}_{{\wrenchnobold}}}
\newcommand{\errortwist}{{\error}_{{\twistnobold}}}
\newcommand{\errorwrenchi}{{\error}_{\wrenchnobold_i}}
\newcommand{\errortwisti}{{\error}_{\twistnobold_i}}

% \newcommand{\errorwrench}{\boldsymbol{\varepsilon}_{\boldsymbol{w}}}
% \newcommand{\errortwist}{\boldsymbol{\varepsilon}_{\boldsymbol{t}}}


\newcommand{\D}{\mathcal{D}}


==> sections/old/0-notation-v1.tex <==
%%% friction for parametric surfaces
\newcommand{\boldsigma}{\boldsymbol{\sigma}}
\newcommand{\boldn}{\boldsymbol{n}}
\newcommand{\boldm}{\boldsymbol{m}}
\newcommand{\surface}{\mathcal{S}}
\newcommand{\tangent}{T_{p}\mathcal{S}}

\newcommand{\pressure}{P}

\newcommand{\vp}{\boldsymbol{v}_p}
\newcommand{\vo}{\boldsymbol{v}_o}
\newcommand{\boldomega}{\boldsymbol{\omega}_\text{IAR}}
\newcommand{\projvp}{\tilde{\boldsymbol{v}}_p}
\newcommand{\boldf}{\boldsymbol{f}}
\newcommand{\boldtau}{\boldsymbol{\tau}}
\newcommand{\boldw}{\boldsymbol{w}}
\newcommand{\boldt}{\boldsymbol{t}}
\newcommand{\boldpredt}{\boldsymbol{\hat{t}}}
\newcommand{\boldW}{\matr{W}}
\newcommand{\disturbance}{\boldsymbol{w}_d}
\newcommand{\wrenchapprc}{\tilde{\boldsymbol{w}}}
%\newcommand{\IAR}{\boldsymbol{\omega}_\text{IAR}}
\newcommand{\contactw}{{\boldsymbol{c}}}
\newcommand{\contactwunit}{\hat{\boldsymbol{c}}}
\newcommand{\fest}{\hat{\boldsymbol{f}}}
\newcommand{\tauest}{\hat{\boldsymbol{\tau}}}
\newcommand{\fperp}{{\boldsymbol{f}_\perp}}
\newcommand{\fperpiunit}{{\hat{\boldsymbol{f}}_{\perp_i}}}
\newcommand{\graspconf}{\boldsymbol{g}}
\newcommand{\state}{\boldsymbol{u}}
\newcommand{\errorwrenchi}{{\varepsilon}_{\boldsymbol{w}_i}}
\newcommand{\errortwisti}{{\varepsilon}_{\boldsymbol{t}_i}}
\newcommand{\errorwrench}{\boldsymbol{\varepsilon}_{\boldsymbol{w}}}
\newcommand{\errortwist}{\boldsymbol{\varepsilon}_{\boldsymbol{t}}}
%\newcommand{\origin}{\mathcal{O}}
\newcommand{\origin}{{\boldsymbol{o}}}
\newcommand{\originx}{{o_x}}
\newcommand{\originy}{{o_y}}
\newcommand{\originz}{{o_z}}


==> sections/old/11-simulations-old.tex <==
\input{figs/figParamSurfaces}
%We evaluate the 6D friction wrench for six non-planar parametric surfaces and compare the wrench error with the discretized surface. 
%Using the parametric surfaces and FEM simulations, we fit the proposed 6DLS models with wrench/twist pairs obtain from a large variety of contact profiles. 
%Finally, physical experiments evaluate the 6DLS-based algorithm for grasp success prediction. 
%We first use synthetic parametric surfaces as contact profiles to examine the 6D friction, surface discretization effect, and the fitting accuracy of the proposed 6DLS.
We first examine the maximal friction wrench for parametric surfaces to show the necessity of 6D friction. 
%An error analysis of friction wrenches is carried out next to analyze the surface discretization effect.  
%The effect of surface discretization is then analyzed by comparing the parametric surfaces
We further evaluate the fitting performance of the proposed 6DLS with a large variety of contact profiles obtained from the parametric surfaces and FEM simulations.

\input{tabs/tableParametricSurfaces}

\input{tabs/tableFrictionParametricSurfaces}



\subsection{Parametric surfaces as contact profile}
\label{subsec:paramSurface}

%\subsubsection{Surface geometry and pressure distribution}
%We use six parametric contact surfaces S1-S6 to evaluate the 6DLS, where Table \ref{tab:parametric_surfaces} summarizes the parametric form of each surface and Fig. \ref{fig:parametric_surfaces} shows the geometries.
We use six contact surfaces S1-S6 to evaluate the 6DLS as illustrated in Fig. \ref{fig:parametric_surfaces}.
Table~\ref{tab:parametric_surfaces} summarizes the parametric form of each surface.
%The parametric form of each surface is in Appendix \ref{app:sub-physical}.
Although the coordinate system can be arbitrarily chosen, we select the axes for S1-S6 so that the contacts are symmetric about the $z$-axis for easier comparison.
We assume the power-law pressure distribution proposed by Xydas and Kao \cite{xydas.1999} to compute the wrenches and twists:
\begin{equation}
	\pressureunit(r) = \pressure_{0} \left[1- \left(\frac{r}{r_{\max}}\right)^k\right]^{1/k}, 
	\label{eq:power}
\end{equation}
where $r_{\max}$ is the maximal distance of a point on the surface to the contact center.
The exponent $k\in \mathbb{R}^+$ controls the shape of the pressure distribution and typically $k \geq 1.8$.
Note that \eq~(\ref{eq:power}) with $k=2$ corresponds to the Hertztian pressure distribution \cite{johnson.1987} and to a uniform distribution with $k=\infty$.
%Two pressure distributions are used for the friction computation: a uniform  and a quadratic pressure distribution, $p_U(r)$ and $p_H(r)$, where $p_H(r)$ approximates the Hertzian model \cite{johnson.1987}: 
$\pressure_{0}$ is a normalization constant so that $\int_\surface \hat{\pressure}(r)=1$.
We select $r$ as the distance to the surface's geometric center $\origin_g$ for S3-S6, while $r$ is the distance to the line parallel to the $z$-axis and goes through $\origin_g$ since the pressure value along the $z$-axis does not vary for S1-S2.
%For S1 and S2, we select $r$ as the distance to the line that is parallel to the $z$-axis and goes through the surface's geometric center $\origin_g$  since the pressure value along the $z$-axis does not vary, while $r$ is selected as the distance to $\origin_g$ for S3-S6.
%For S1 and S2, the contact center is a line that is parallel to the $z$-axis and goes through the geometric center since the pressure value along the $z$-axis does not vary, when e.g. a deformable jaw is grasping a rigid cylinder. 





\subsection{Maximal friction wrench for parametric surfaces}
Table \ref{tab:wrench_parametric_surface} shows the maximal friction in each dimension for the six surfaces.
We select a uniform pressure distribution and $\mu=1$ to better compare $\vec{f}$ and $\vec{\tau}$ of different geometries. 
%$f_{x,y,z}$ reach the maximum when the angle between $\vec{f}$ at each point and the positive $x,y,z$-axis is minimal, respectively.
{\color{crev1}$f_{x,y,z}$ reaches the maximum when $\vec{f}$ at each point is closest to parallel to the  $x,y,z$-axis, respectively, which is equivalent to projecting the axis onto the tangent plane at each point.
Therefore, $f_{{x_\text{max},y_\text{max},z}_\text{max}}$ can be computed by substituting $\vt$ in \eq~(\ref{eq:projvp}) with the respective negative axis and computing $\vec{f}$ with \eq~(\ref{eq:frictionArea}).
For S1 and S2, $f_{z_\text{max}}$ equals one since there is no curvature along the $z$-axis.
For S1, S3, S5, $f_{x_\text{max}}$ and $f_{y_\text{max}}$ are equal because the integral of the projected $x$- and $y$-axis are the same. }
%Take $S1$ as an example.
%Denote $F$ as the magnitude of frictional force at each point, $f_{x_{\text{max}}} = F\int_0^\pi  \sin u \diff u = F\int_0^{\pi/2}  (-\cos u) \diff u + F  \int_{\pi/2}^\pi  (-\cos u) \diff u = f_{y_{\text{max}}}$.
{\color{ceditor}Assuming a planar contact area in the $xz$-plane  or only considering the 3D friction for curved surfaces in previous work \cite{xu.2017} lead to the maximum of $f_y$, $\tau_x$, and $\tau_z$  being 0, resulting in an over-conservative model in the 3D subspace. 
The former assumption also results in $f_{x_\text{max}}=1$ and $f_{z_\text{max}}=1$ for all surfaces, which is an overconfident estimation for $f_x, f_z$, and $\tau_y$. 
Comparing these values with Table~\ref{tab:wrench_parametric_surface} shows the necessity of the proposed 6D friction model.}
 
%Similar to planar contacts, the maximal torque computed with the Hertzian pressure distribution is smaller than with the uniform distribution.% when the contact center is near the pressure-weighted friction center. 

\input{figs/figDiscretizationEffect}

\input{figs/figLSParametricSurfaces}




\subsection{Surface discretization effect}
\label{sec:discretizationEffect}


%The friction is then computed by summing up the contribution of each small element. 
We also analyze the difference in the friction wrench between the parametric and the meshed surfaces for S1-S6  with 25-1000 triangular elements.
We compute the maximal friction wrench in each dimension with the power-law pressure distribution with $k=\infty$ and consider the wrench obtained by the parametric surfaces as the ground truth. 
The wrench differences are divided by the ground truth and averaged over all dimensions, defined as the wrench error rate.
{\color{crev3}As shown in \fig~\ref{fig:discretizationEffect}, the error of all surfaces rapidly decreases with the number of elements since the meshed surfaces are closer to the parametric ones and is below 4\% with 300 triangles, which is acceptable in most applications and is nearly zero with 1000 elements.}
S1, S2 have the lowest error since there is no curvature along the $z$-axis.
Next, we measure the runtime on an Ubuntu 16.04 machine with an Intel Core i7-8700K CPU (3.7 GHz) with a MATLAB implementation without parallel computing or GPU acceleration. 
While the average runtime to integrate a single wrench is 2.62s, the computation for a discrete surface requires 1.3ms and achieves a 2000x speedup. 


\input{figs/figLSExamples}

\input{figs/figFEM}

\subsection{6DLS evaluation with parametric surfaces}

\label{seq:Fitting_results_parametric_surface}
\mysum{LS visualization}

We evaluate the fitting results of the 6DLS with different numbers of filtered wrench and twist pairs obtained from the parametric surfaces and two pressure distributions: $k=2$ and $k=\infty$.
%The six parametric surfaces with uniform and Hertzian pressure distribution are used as the contact profile. 
%We densely sample the IARs for each contact profile and obtain around 40000 wrench and twist pairs, which are then evenly down-sampled to fit the 6DLSs. 
We select the weight for the wrench and twist error  $\weight_1 = 10, \weight_2 = 1$ since we use approximated twists (as described in Section~\ref{sec:sampling_IAR}).
\fig~\ref{fig:lsErrorParametricSurface}(a) and (b) show the mean error of wrenches and twists, the error is computed with all 40000 samples before filtering.
\fig~\ref{fig:lsErrorParametricSurface}(c) illustrates the corresponding runtime. 
Fitting a quartic model is slower since it has 126 variables while the ellipsoid has 21.
We observe that the error of the quartic 6DLS rapidly decreases with a higher number of samples and yields better results with more than 50 pairs.
An appropriate LS model can be selected based on the trade-off between the fitting error and the runtime required by the application. 


%\input{sections/tableLSParametricSurfaces}

\fig~\ref{fig:LSExamples} shows an representative 3D cross-section of the quartic and ellipsoidal 6DLS with enlarged views of wrenches and twists, where the other three components are 0.
Each LS is fit to 300 pairs obtained from S4 (ellipsoid) with a uniform pressure distribution. 
Orange dots indicate wrenches, while the green and purple arrows illustrate the corresponding twists and predicted twists (surface normal at each wrench), respectively.
Results suggest that the quartic 6DLS is a better fit, since most wrenches are on its surface, the angle differences between the fitting and the predicted twists are smaller.

%Fig. \ref{fig:LS4th} and Fig. \ref{fig:LS2nd} 
%Each figure shows 20 three-dimensional cross-sections of the 6D model, where the other three components are 0.






%\input{sections/figDBParameters}

\subsection{6DLS evaluation with FEM simulations}

\mysum{The results here are for individual contact, since they are different source of the contact information}
\label{subsec:FEM}

%Next, we evaluate the 6DLS models with larger varieties of surfaces and pressure distributions. 
%The contact profiles are obtained from the FEM simulation between deformable objects and a parallel gripper, which is mounted with two types of soft finger.
%The objects are generated based on the synthetic dataset of thin-walled deformable objects from our previous work \cite{alt.2016}. 
%We use the commercial FEM simulation software ANSYS \textregistered \cite{ansys}, which provides a high-quality meshing tool and the shell element type that is suitable for thin-walled objects, such as plastic bottles. 

We use FEM simulation to generate large varieties of contact profiles including the contact surfaces and pressure distributions.
The wrench and twist pairs calculated from the profiles are used to evaluate the fitting accuracy of the proposed 6DLS.

We simulate contacts between a parallel jaw gripper and deformable thin-walled objects using a commercial software ANSYS \cite{ansys} based on our previous work \cite{alt.2016}. 
The object geometry is described with non-uniform rational B-Splines (NURBS), which is then meshed according to quality preferences.
%Details regarding the NURBS geometry generator and locations of antipodal grasps can be found in Appendix~\ref{sec:sub-FEM}.
%We describe the object models with non-uniform rational B-Splines (NURBS) and use a commercial software ANSYS \cite{ansys} for the simulations, which provides a high-quality meshing tool and accurate simulation results.
%The objects are generated based on the synthetic dataset of thin-walled deformable objects from our previous work \cite{alt.2016}. 
The top of Fig. \ref{fig:FEM_sim}(a) depicts the parametric generation of the geometry. 
An ellipse defines the base and a spline curve shape the wall, which is controlled by variables $p_{1\ldots12}$.
We then vertically sample the curve and create an ellipse at each sample, where adjacent ellipses rule the object surface, as illustrated in Fig.~\ref{fig:FEM_sim}(a) bottom.
The squares and circles mark the locations of antipodal grasps with two approach directions.
By varying parameters $p_{1\ldots12}$, we efficiently generate 24 objects for simulation, as shown in Fig. \ref{fig:FEM_sim}(b).


 \input{tabs/tableFrictionFEM}

%Here, we briefly describe the model generation from our previous work \cite{alt.2016} and the smooth surface generation in this work.  
%The object geometries are generated based on real-life objects. 

%generate a dataset with different object geometries.
%For a smooth surface generation, ellipses are first created at each sample, which are visualized as $E_{1,\ldots,n}$ in Fig.~\ref{fig:db_parameters}(b).
%The surface of the object is then ruled by adjacent ellipses. 
%Numerous objects with different geometry can be efficiently created by various combinations of the parameters. 
%We use 24 objects for simulations, as shown in Fig. \ref{fig:fem_objects}, where object 17-24 are asymmetric. 
We use two types of deformable jaws for simulations: the top of Fig.~\ref{fig:FEM_sim} (c) depicts the beam-shaped jaws, while the bottom illustrates the ellipsoidal fingertips.
While the former mimics contacts with the Festo Fin-Ray\textregistered \ deformable plastic jaws \cite{festo}, the latter simulates biologically-inspired fingertips such as the SynTouch BioTech\textregistered \cite{syntouch}.
We simulate contacts at each grasp location with five normal forces in the range of 2-13N, resulting in 2473 total contacts. 
%The antipodal grasp locations are illustrated in Fig.~\ref{fig:db_parameters}(b) with square and circle pairs for two approach directions.
%Fig.~\ref{fig:FEM_sim}(a) and (b) show the beam-shaped jaws before and after applying the pressure load. 
%Such finger is selected to mimic the contact of the deformable plastic fingers, e.g. the Festo Fin-Ray\textregistered \ gripper jaws \cite{festo}. 
%Fig.\ref{fig:FEM_sim}(c) and (d) illustrate the simulation with ellipsoidal tips, which mimic biologically-inspired jaws such as the SynTouch BioTech\textregistered \cite{syntouch}. 
%For each grasp location, five forces with the magnitudes 2N, 5N, 7N, 10N, 13N are applied perpendicular to the fingers by adding the pressure load. 
%We simulate contacts at each grasp location with five normal forces range from 2-13N and results in total 2473 contacts. 



We compute 150 wrenches and twists for each contact. 
Table \ref{tab:FEM} summarizes the mean and the standard deviation of the fitting error with the two 6DLS models. 
%We compute 150 wrenches and twists for each contact and the Table \ref{tab:FEM} shows the performance of the 6DLS models.
%Table \ref{tab:FEM} shows the performance of the 6DLS models fitted with 150 wrenches and twists obtained from each contact. 
%%We obtained in total 2473 contacts from the simulation.
%For each contact, we compute the possible wrenches and twists and down-sample to 150 pairs for the limit surface fitting. 
%The mean and standard deviation (std) of the fitting error of that both LS models are shown in Table \ref{tab:FEM}.
The quartic model yields a lower error.
Since both gripper types have similar errors, the results suggest that the proposed 6DLS models are suitable for a large variety of contact profiles. 
% or are not restricted by certain contact geometry or pressure distribution. 









==> sections/old/5-problem-statement-twist.tex <==
%\subsection{Overview}
We consider the problem of modeling the frictional force and torque of a non-planar surface contact with a 6D limit surface. 
We further apply the limit surface of each contact to predict binary success of multi-contact grasps with deformable gripper jaws.


\subsection{Assumptions}
%The assumptions are summarized as follows:
\begin{enumerate}
%	\item {\color{ceditor}Quasi-static physics (inertial terms are negligible) and Coulomb's friction with a known constant coefficient of friction.} 
	\item {\color{ceditor}Coulomb friction with a known constant coefficient of friction.} 
	\iten Quasi-static physics because xxx 
%	\item The object is not caged.
%	\item The change of the contact surface and the pressure distribution that is caused by the friction is neglected. 
	\item {\color{ceditor}Geometry and pressure distribution of the contact interface or their estimations are known and remain constant during the grasp.}

%	The normal pressure and tangential friction is typically treated separately since the influence of the tangential friction upon the normal pressure is small \cite{johnson.1987}.
\end{enumerate}


\subsection{Definitions and notation}
\mysum{Notation for a parametric surface}
We adapt the notation from \cite{pressley.2010.elementary,howe.1996,murray.2017}: 
%$\surface$: a surface. \\
\begin{itemize}
%	\item $\boldsigma(u,v) = [\sigma(u,v)_x, \hspace{0.2em}\sigma(u,v)_y,\hspace{0.2em}\sigma(u,v)_z]^T, \hspace{0.2em}(u,v)\in \mathbb{R}^2$: the parametrization of the surface $\surface$. 	
%	\item $\boldsigma _{u,v}$: the first-order derivative of $\boldsigma$ with respect to $u,v$, respectively. 	
	%$\boldsigma _v$: the first-order derivate of $\boldsigma$ with respect to $v$. \\
%	\item $p$: a point on the surface $\surface$ with the parametric form  $\boldsigma(u_p,v_p)$, where $p \in \surface$.	
%	\item $\tangent$: the tangent plane of a surface $\surface$ at a point $p \in \surface$.	
%	\item $\boldn_p$: the surface normal at point $p$.	
	%\item $dA$: area of a small parallelogram.
%	\item $\boldsymbol{\origin}$: the origin of the contact.  
	%$\lcor$: the center of rotation (COR) axis, which is line in 3-dimensional space. \\
	%$\boldomega$: the angular velocity \\	

	\item $\boldomega$: the instantaneous axis of rotation (IAR) of a body with direction $\boldsymbol{m}$ that goes through the point $\boldsymbol{r}_o$
	\item $\surface$: the contact surface	
	\item $\fperp\in \mathbb{R}^3$: the normal force of a contact
	\item $\pressure$: the pressure distribution with $\int_\surface \pressure = \norm{\fperp}$	
	\item $\pressureunit$: the unit pressure distribution with $\int_\surface \pressureunit = 1$	
%	\item $\vp$: the linear velocity at point $p$.	
%	\item $\projvp$: the relative linear velocity at point $p$, which lies in the tangent plane  $\tangent$.	
%	\item $\pressure(u_p,v_p)$: the pressure at the point $p$.	
	\item $\mu$: the coefficient of friction 	
%	\item $\boldsymbol{\origin}$: the friction-weighted center of pressure
	\item $\boldf = [f_x,f_y,f_z]^T$: the frictional force	
	\item $\boldtau = [\tau_x,\tau_y,\tau_z]^T$: the frictional torque 	
	\item $\wrench = [f_x,f_y,f_z,\tau_x,\tau_y,\tau_z]^T$: the friction wrench 
	\item $\twist \in \mathbb{R}^6$: the unit twist of the grasped object
	\item $\twistrel \in \mathbb{R}^6$: the relative twist between the grasped object and the gripper jaw

	\item $\predt \in \mathbb{R}^6$: the predicted relative twist at the contact	
	\item $\W = \left\{\hat{\wrench}_{i\in\{\{1 \ldotsc P\}} ,\hat{\twist}_{i\in\{\{1 \ldotsc P\}} \right\}$: the set of $P$ normalized wrench and twist pairs to fit the 6DLS models
	\item $\A$: the limit surface model fit to wrench and twist pairs
	\item $\Ae$: the ellipsoidal limit surface model
	\item $\Aq$: the quartic limit surface model 
	\item $\D$: the dataset of limit surface models $\A$
	\item $\errorwrench$: the limit surface fitting error of wrenches
	\item $\errortwist$: the limit surface  fitting error of twists
\end{itemize}

The  integral of a 3D vector function is defined as three individual integrals of each component \cite{howe.1996}: 
%This means that the integral of the vector $\boldsymbol{v} = [v_x,v_y,v_z]^T$ is defined as: 
\begin{align*}
	\boldsymbol{V} = \begin{bmatrix} {V_x}\\{V_y}\\{V_z} \end{bmatrix}= \int \boldsymbol{v} \diff{t} =  \begin{bmatrix}{\int v_x \diff{t}}\\{\int v_y \diff{t}}\\{\int v_z \diff{t}} \end{bmatrix} \text{, with } \boldsymbol{v} = \begin{bmatrix}{v_x}\\{v_y}\\{v_z}\end{bmatrix}.
\end{align*}

\subsection{Metrics}
\label{sec:metrics}
We evaluate the 6D limit surface models with fitting error of wrenches $\errorwrench$ and twists   $\errortwist$.
While $\errorwrench$ is measured with the mean distance of wrenches to the LS,  $\errortwist$ is the mean angle between $\boldt$ and $\boldpredt$.

Additionally, we apply the proposed 6DLS to predict multi-contact grasp success. 
We consider a grasp to be successful if it lifts the object and there is no relative motion between the object and gripper jaws and a failure otherwise.
%A binary function $R$ describes the grasp success, where $R=1$ if the grasp lifts the object and there is no relative motion between the object and gripper jaws and $R=0$ otherwise.
We seek to maximize precision and recall of binary predictions on physical experiments.
Denote $tp$ as the number of true positive predictions, $fp$ as false positives, and $fn$ as false negatives,  precision is calculated as $tp/(tp+fp)$ and recall is computed by $tp/(tp+fn)$. 
A combination of high precision and recall indicates that the algorithm predicts few false positives and false negatives.
Both metrics are commonly used for datasets with unequal class distributions in computer vision and can describe if the algorithm is overconfident or too conservative~\cite{everingham2010pascal}.











==> sections/old/6-friction-param-surface-twist.tex <==
The algorithm to compute friction wrench for non-planar surfaces is similar to planar contacts \cite{goyal.1991,howe.1996,mason2001mechanics}, a theoretical background can be found in Appendix \ref{appendix:background}.
We assume a known instantaneous motion of the grasped object and compute the contact velocity and the friction wrench at each point on the contact surface. 
The integral of the local friction contribution forms the total friction wrench of the contact surface. 
We then sample many instantaneous body motions to obtain possible friction wrenches of the contact surface. 
For a representative grasp as shown in \fref{fig:headshot}, we compute friction wrenches of the contact surface between the left jaw and the rigid cup by sampling many instantaneous motions of the cup. 
Note that the motion considered in this work is the "virtual motion", or the motion tendency of the grasped object.
We start with formulating the instantaneous body motion, followed by determining the frictional force and torque given a motion for a parametric or a discrete surface. 
% Assuming a known instantaneous body twist, we compute the relative velocity and the friction wrench at each point on the contact surface. 
% The integral of the local friction contribution forms the total friction wrench of the surface.
% We then sample many twists to obtain possible friction wrenches.

%Coulomb friction states that the direction of the frictional force is opposed to the relative velocity.
%We compute the friction wrench by assuming a known relative velocity at each point, then integrating the friction contribution of each point on the surface. 
%Sampling relative velocities provides possible friction wrenches.
%However, the relative velocity is nontrivial to sample. 
%It depends on the instantaneous body motion and the contact geometry, since the velocity at a point on the surface is tangential to this point. 
%Therefore, we assume a known instantaneous body twist and compute the relative velocities. 
%We then sample many twists to obtain multiple velocities at each point.

\subsection{Formulation of the Instantaneous Body Motion}
\label{subsec:twist}
The instantaneous body motion in three dimensions, or \emph{twist}, is the combination of a translation along an axis and a rotation about the same axis, defined as the \emph{instantaneous screw axis} (ISA). 
This means the linear velocity $\vel~\in~\R{3}$ is the sum of a velocity parallel to and a velocity perpendicular to the ISA, denoted as $\vpara$ and $\vperp$, respectively. 
Adapted from~\cite{murray.2017}, we represent the ISA as a directed line $\lineISA$ though a point $\linepoint~\in~\R{3}$, with the unit vector $\linedir~\in~\R{3}$ specifying the direction.
Denoting $\boldomega~\in~\R{3}$ as the angular velocity with $\boldomega=\normang\linedir$ and $h~\in~\mathbb{R}$ as the ratio of translational to rotational motion, or the scalar pitch, we compute $\vel$ with %We then compute the linear velocity $\vel~\in~\R{3}$ as the sum of the velocities that are parallel and perpendicular to $\lineISA$, denoted as $\vpara$ and $\vperp$, respectively:
\begin{equation}
\vel = \vpara + \vperp = h \boldomega + \linepoint \times \boldsymbol{\omega} = \normang \left( h \linedir + \linepoint \times \linedir \right).
\label{eq:velocity}
\end{equation}
% The twist $\twist~\in~\R{6} $ is defined as
% \begin{equation}
% \twist = \begin{bmatrix}{\vel}\\{\boldomega}\end{bmatrix} = \norm{\boldomega}\begin{bmatrix}{h \linedir + \linepoint \times \linedir}\\{\linedir}\end{bmatrix}.
% \label{eq:twist}
% \end{equation}
A twist is defined as $\left[\vel^T,\boldomega^T \right]^T$. A twist is a pure rotation about $\lineISA$ if $\norm{\boldsymbol{\omega}} \neq 0$ and $h=0$, a pure translation along $\lineISA$ if $\norm{\bolsdsymbol{\omega}} = 0$ and $h=\vel^T \boldomega / \norm{\boldomega}^2=\infty$. 
Since the magnitude of $\angular$ or $\vel$ does not affect the friction wrench under Coulomb friction, we define the \emph{unit twist} $\twist\in \R{6}$ that is a twist with $\norm{\boldomega}=1$, or $\norm{\boldomega}=0$ and $\norm{\vel}=1$, adapted from~\cite{murray.2017}
\begin{equation}
 \twist =  
\begin{dcases*}
\begin{bmatrix}{h\linedir +\linepoint\times \linedir} \\ {\linedir} \end{bmatrix}& 
if $ \normang=1$\\
\begin{bmatrix}{\linedir} \\ {\boldsymbol{0}} \end{bmatrix} &if $ \normang=0$. 
\end{dcases*}
\label{eq:twist}
\end{equation}
% By sampling many unit twists of the grasped object, we compute the linear velocity at each point on the contact surface and thus the friction wrench. We then use the wrench and twist pairs to fit the limit surfaces as described in \sref{sec:LS}.
We use the linear velocity of $\twist$ to compute friction wrench in the following section and fit the limit surface models using wrench and twist pairs by sampling many unit twists, as described in \sref{sec:LS}.

\begin{figure}[!t]
	\centering
	{{\includegraphics[width=85mm,trim={4.1cm 14cm 3cm 6cm}, clip]{figs/sources/curved-friction-nop.pdf} }}% 
	\caption{\small Friction computation for a non-planar parametric contact surface $\surface$. Assuming a known instantaneous screw axis $\lineISA$, we compute the linear velocity $\vel$ for each point $\boldsigma(u,v) \in \surface$ and the relative velocity $\vr$ by projecting $\vel$ onto the tangential plane. The local frictional force $\diff \boldsymbol{f}$ is antiparallel to $\vr$. The integral of the local frictional force and torque forms the friction wrench of  $\surface$.}
	\label{fig:curved-friction}
\end{figure}

\subsection{Friction Formulation for a Parametric Surface}
\label{subsec:frictionParametricSurface}
Given a unit twist of the grasped object described with the ISA $l$ and the pitch $h$ that is finite, we compute the linear and the relative velocity at each point on the contact surface $\surface$. The frictional force at each point is antiparallel to the relative velocity at that point. 
\fref{fig:curved-friction} depicts the derivation of the local frictional force on $\surface$ given $l$ and $h$.

Denoting $\boldsigma(u,v)$ as the parametric form of $\surface$, with $(u,v)~\in~\mathbb{R}^2$ being the coordinate,  the linear velocity $\vel$ at $(u,v)$ is
\begin{equation}
 \velfunc =  
\begin{dcases*}
h\linedir + \left(\linepoint -\boldsigma(u,v)\right) \times \linedir & 
if $ \normang=1$\\
\linedir &if $ \normang=0$. 
\end{dcases*}
\label{eq:velocity}
\end{equation}

% Based on $\velfunc$, we determine the relative velocity $\vrfunc$ that is tangential to $\surface$ at $(u,v)$. 
The relative velocity $\vrfunc$ is tangential to $\surface$ at $(u,v)$. 
Let $\boldsigma _u$, $\boldsigma _v$ be the first-order derivatives of $\boldsigma(u,v)$ with respect to $u$ and $v$, respectively. The surface normal of the tangent plane of $\surface$ is  $\normal={\boldsigma _u \times \boldsigma _v}/{\norm{\boldsigma _u \times \boldsigma _v}}$. Denoting the scalar projection $\scalar=\vel^T \normal$, we compute $\vr$ by projecting $\vel$ onto the tangent plane

\begin{equation}
\vrfunc = \frac{\velfunc - \scalarfunc \bigcdot \normalfunc }{\norm{\velfunc - \scalarfunc \bigcdot \normalfunc}}.
\label{eq:projvp}
\end{equation}


The local frictional force $\diff\boldf$ is antiparallel to $\vr$. Denoting $\pressure(u,v)$ as the pressure distribution of $\surface$, $\diff\boldf$ is computed with $\diff\boldf = -\mu \bigcdot \pressure \bigcdot \vr \bigcdot\norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}$. 
We then determine the frictional torque with respect to the pressure center $\boldsymbol{\origin}$, which is 
\begin{equation}
\begin{aligned}
\boldsymbol{\origin} = \begin{bmatrix}{\originx}\\{\originy}\\{\originz}\end{bmatrix} &= \frac{\int_ \surface \boldsigma(u,v)  \bigcdot \pressure(u,v) \bigcdot\norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}}{\int_ \surface  \pressure(u,v)\bigcdot \norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}}.
\end{aligned}
\end{equation}
Note that $\origin$ may not be on the contact surface. 
With the torque arm $\arm = \boldsigma(u,v) - \boldsymbol{\origin}$, the local frictional torque $\diff\boldtau$ is $\diff\boldtau =  \arm \times \diff\boldsymbol{f}$.
By integrating the frictional contribution at each point, the frictional force and torque of  $\surface$ for a given unit twist is 
\begin{equation}
\begin{aligned}
\boldf &= - \int _\surface   \mu \bigcdot \pressure(u,v) \bigcdot  \vrfunc \bigcdot\norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}  \\ 
\boldtau &=  - \int _\surface \mu \bigcdot \pressure(u,v) \bigcdot [\arm(u,v)  \times \vrfunc] \bigcdot\norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}.
\end{aligned}
\label{eq:frictionArea}
\end{equation}


% Knowing the extrema of the frictional force and torque is beneficial to construct a limit surface.
% Similar to \cite{howe.1996}, we analyze the extrema by considering the twists.
% Note that different unit twists may lead to an identical friction wrench due to the surface geometry constraints. 
% $f_x$ is maximal when the twist is a pure translation along the $x$-axis.
% $\tau_x$ is maximal when the IAR is parallel to the $x$-axis and goes through $\boldsymbol{\origin}$ since the torque arm is then closest to perpendicular to the frictional force at each point.



==> sections/old/6-friction-param-surface_ori_formulation.tex <==
The algorithm to compute friction for non-planar surfaces is similar to planar contacts \cite{goyal.1991,howe.1996}.
A theoretical background can be found in Appendix \ref{appendix:background}.

Coulomb's friction model states that the direction of the frictional force is opposed to the relative velocity.
We compute the friction wrench by assuming a known relative velocity at each point, then integrating the friction contribution of each point on the surface. 
Sampling relative velocities provides possible friction wrenches.
%By sampling different relative velocities, we obtain possible friction wrenches of a contact.  
\mysum{why sampling IAR}
However, the relative velocity is nontrivial to sample. 
It depends on the instantaneous body motion and the contact geometry, since the velocity at a point on the surface is tangential to this point. 
Therefore, we assume a known instantaneous body twist and compute the relative velocities. 
We then sample many twists to obtain multiple velocities at each point.

\subsection{Formulation for a parametric surface}
\label{subsec:frictionParametricSurface}

\mysum{The general idea}
%In this section, we describe the friction computation for a three-dimensional contact surface with a known parametric form, a pressure distribution, and a coefficient of friction.

\fig~\ref{fig:curved-friction} depicts the derivation of the friction wrench for a point $p$ on the contact surface $\surface$ with a given twist.
%We start with the parametrization of a body twist. 
A twist consists of a velocity ($\boldsymbol{v}_{\perp}$) perpendicular to the instantaneous axis of rotation $\boldomega$ and a linear velocity ($\boldsymbol{v}_{\parallel}$) parallel to $\boldomega$.
We parametrize the IAR as a line with direction $\boldm$ that goes through a point $\boldsymbol{r}_o$:
%\begin{align}
%	\lIAR &= \boldsymbol{r_o} + \boldomega \bigcdot t \\
%	&= [r_{o_x},r_{o_y},r_{o_z}]^T + [\omega_x,\omega_y,\omega_z]^T \bigcdot t
%\end{align}
\begin{equation}
	\boldomega = \boldsymbol{r}_o + \boldm \bigcdot t \text{, with } \norm{\boldm} = 1,t \in \mathbb{R}. 
	\label{eq:IAR}
\end{equation}

\mysum{Parametrization of a surface}
%The velocity of each point on the surface is computed given the  $\boldsymbol{\omega}$.
We denote $\boldsigma(u,v)$ as the parametric form of $\surface$ with $(u,v)~\in~\mathbb{R}^2$ and  $\boldsigma(u_p,v_p)$ as the parametric form of a point $p \in \surface$.
\mysum{Velocity computation}
Denoting $h$ as the screw pitch, the velocity $\vp$ at $p$ is computed with: 
%The velocity $\vp$ at $p$ is computed based on \eq~(\ref{eq:twist}): 
\begin{equation}
\begin{aligned}
\vp &= \boldsymbol{v}_{p_{\parallel}} +\boldsymbol{v}_{p_\perp}, \\ 
& = h \bigcdot \boldm + (\boldsigma(u_p,v_p) - \boldsymbol{r}_o) \times \boldm.
\end{aligned}
\label{eq:velocity}
\end{equation}
$\tangent$ is the tangent plane of $\surface$ at $p$ with the normal $\hat{\boldn}_p$, and $\boldsigma _u$, $\boldsigma _v$ are the first-order derivatives of $\boldsigma(u,v)$ with respect to $u$ and $v$, respectively.
The relative velocity $\projvp$ is the projection of $\vp$ onto $\tangent$:
%\begin{equation}
%\begin{aligned}
%	\projvp &= \vp - \frac{\vp^T \boldn_p}{\norm{\boldn_p}^2} \bigcdot \boldn_p \text{, with } \\
%	\boldn_p &= \frac{\boldsigma _u \times \boldsigma _v}{\norm{\boldsigma _u \times \boldsigma _v}}.
%\end{aligned}
%\label{eq:projvp}
%\end{equation}
{\color{crev2}
\begin{equation}
\begin{aligned}
\projvp &= \frac{\vp - c_p \bigcdot \hat{\boldn}_p }{\norm{\vp - c_p \bigcdot \hat{\boldn}_p }} \text{, with } \\
\hat{\boldn}_p &= \frac{\boldsigma _u \times \boldsigma _v}{\norm{\boldsigma _u \times \boldsigma _v}}, c_p=\vp^T \hat{\boldn}_p.
\end{aligned}
\label{eq:projvp}
\end{equation}
}

\begin{figure}[!t]
	\centering
	{{\includegraphics[width=85mm,trim={4.1cm 14cm 3cm 6cm}, clip]{figs/sources/curved-friction.pdf} }}% 
	\caption{Friction computation for a non-planar parametric contact surface $\surface$. Assuming a known instantaneous axis of rotation ($\boldomega$), we compute the velocity $\boldsymbol{v}_p$ at a point $p$ and the relative velocity $\tilde{\boldsymbol{v}}_p$ by projecting $\boldsymbol{v}_p$ onto the tangential plane $\tangent$. The frictional force $\boldsymbol{f}_p$ at $p$ is antiparallel to $\tilde{\boldsymbol{v}}_p$. The integral of the friction contribution at each point forms the friction of  $\surface$.}
	\label{fig:curved-friction}
\end{figure}

%Finally, the projected velocity $\projvp$ at point $p$ is computed by: 
%\begin{equation}
%	\projvp = \vp - \frac{\vp \bigcdot \boldn_p}{\norm{\boldn_p}^2} \bigcdot \boldn_p.
%	\label{eq:projvp}
%\end{equation}

\mysum{Friction computation}
Based on $\projvp$, the friction at $p$ can now be computed with respect to the friction-weighted center of pressure $\boldsymbol{\origin}$ of $\surface$:
{\color{ceditor}
\begin{equation}
\begin{aligned}
\boldsymbol{\origin} = \begin{bmatrix}{\originx}\\{\originy}\\{\originz}\end{bmatrix} &= \frac{\int_ \surface \boldsigma(u,v)  \bigcdot \pressure(u,v) \norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}}{\int_ \surface  \pressure(u,v) \norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}}.
\end{aligned}
\end{equation}
}
%where:
%\begin{equation}
%	\diff{A} = \norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}.
%\end{equation}
%Note that the origin $\boldsymbol{\origin}$ might not be on the surface $\surface$.

%\begin{equation}
%	\begin{aligned}
%		d\boldf_p &=  -  \mu \bigcdot \pressure(u_p,v_p) \bigcdot  \frac{\projvp}{\norm{\projvp}} \diff{\surface}, \\ 
%		d\boldtau_p &=  \boldsymbol{l}_p \times d\boldsymbol{f}_p \text{, where } \\
%		\boldsymbol{l}_p &= \boldsigma(u_p,v_p) - \boldsymbol{\origin}.
%	\end{aligned}
%	\label{eq:frictionPoint}
%\end{equation}

The local frictional force $d\boldf_p$ at $p$ is opposed to $\projvp$ and $d\boldf_p = -\mu \bigcdot \pressure(u_p,v_p) \bigcdot  \projvp \diff{A}$.
The local frictional torque at $p$ is $d\boldtau_p =  \boldsymbol{l}_p \times d\boldsymbol{f}_p$ with the torque arm $\boldsymbol{l}_p = \boldsigma(u_p,v_p) - \boldsymbol{\origin}$.
By integrating the frictional contribution at each point, the friction of  $\surface$ for a given body twist is determined by:
\begin{equation}
\begin{aligned}
\boldf &= - \int _\surface   \mu \bigcdot \pressure(u,v) \bigcdot  \projvp \norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v},  \\ 
\boldtau &=  - \int _\surface \mu \bigcdot \pressure(u,v) \bigcdot [\boldsymbol{l}_p  \times \projvp] \norm{\boldsigma_u \times \boldsigma_v}  \diff{u} \diff{v}.
\end{aligned}
\label{eq:frictionArea}
\end{equation}

%By substituting equation (\ref{eq:velocity}) - (\ref{eq:frictionPoint}) into equation (\ref{eq:frictionArea}), the friction wrench can be computed by $\boldw = [\boldf^T,\boldtau^T]^T$.
Knowing the extrema of the frictional force and torque is beneficial to construct a limit surface.
Similar to \cite{howe.1996}, we analyze the extrema by considering IARs.
Note that different IARs may lead to an identical friction wrench due to the surface geometry constraints. 
Typically, $f_x$ reaches the maximum when the IAR is parallel to the $y$-axis and infinitely far away along the $z$-axis or when it is parallel to the $z$-axis and infinitely far away along the $y$-axis. 
$\tau_x$ is maximal when the IAR is parallel to the $x$-axis and goes through $\boldsymbol{\origin}$ since the torque arm is then closest to perpendicular to the frictional force at each point.
%Similarly, the extrema can be obtained for $f_{y,z}, \tau_{y,z}$. 

%Possible friction wrench data are obtained by sampling the IAR. 
%Sampling strategy is described in Section. \ref{sec:sampling_IAR}.


==> sections/old/7-friction-discrete-surface-twist.tex <==
\subsection{Friction formulation for a discrete surface}
\label{subsec:frictionDiscreteSurface}
%The parametric form of a surface is not always available, e.g. when the contact is obtained from an FEM simulation. 
%We focus on discrete surfaces with triangular elements in the following, which can be easily extended to other polygonal elements. 
The computation for a parametric surface is typically less efficient than for a discrete one since the runtime for an integral is slower than for a sum operation. 
In the following, we compute friction wrench for discrete surfaces with $N$ convex polygonal elements.

Consider the $i$-th element with the center $\centeri$ and the normal $\normali,i=1,\ldots,N$, we compute the relative velocity $\vri$ at $\centeri$ given a unit twist parametrized as in \eref{eq:twist}
 %with 	\ref{eq:projvp} equation, where:
\begin{equation}
	\begin{aligned}
	 &\vel_i =  
    \begin{dcases*}
    h\linedir + \left(\linepoint -\centeri\right) \times \linedir & 
    if $ \normang=1$\\
    \linedir &if $ \normang=0$
    \end{dcases*} \\
	&\vri = \frac{\vel_i - \scalar_i \normali}{\norm{\vel_i - \scalar_i \normali}} \text{ with }   \scalar_i= \frac{\vti^T \normali}{\norm{\normali}^2}.
	\end{aligned}
\end{equation}

Denoting  $\pressurei$ and $\areai$ as the pressure and the area of the $i$-th element, respectively, the pressure center $\boldsymbol{\origin}$ of the surface is
\begin{equation}
\begin{aligned}
\boldsymbol{\origin} = \begin{bmatrix}{\originx}\\{\originy}\\{\originz}\end{bmatrix}= \frac{\sum_ {i=1}^N \centeri \bigcdot \pressurei \bigcdot \areai}{\sum_ {i=1}^N  \pressurei \bigcdot \areai}. 
\end{aligned}
\end{equation}

The frictional force and torque of the discrete surface is:
\begin{equation}
\begin{aligned}
\boldsymbol{f} &= -\sum_{i=1}^N \mu \bigcdot \pressurei \bigcdot \areai \bigcdot \vri  \\
\boldsymbol{\tau} &= -\sum_{i=1}^N \mu \bigcdot \pressurei \bigcdot \areai \bigcdot [(\centeri- \boldsymbol{\origin}) \times \vri].
\end{aligned}
\label{eq:frictionDiscrete}
\end{equation}

We analyze the runtime and the error of friction wrench due to the surface discretization in Section~\ref{sec:discretizationEffect}.

==> sections/old/8-limit-surface-twist.tex <==
\section{Six-dimensional Limit Surface}
\label{sec:LS}
In this section, we study the problem of what friction wrenches can be transmitted through a non-planar surface contact by finding a 6D limit surface. 
We start with the definition of the LS, followed by finding wrench and twist pairs to fit two LS models, generalized from 3D models that are widely used for planar surface contacts: an ellipsoidal mode \cite{howe.1996} and a convex fourth-order polynomial model (the quartic model) \cite{jiaji.2016}. 

\subsection{Definition and Properties}
A limit surface is the boundary of the set of all possible friction wrenches that can be applied through one contact or a set of contacts \cite{goyal.1991}.
% The surface is closed, convex, and encloses the origin of the wrench space. 
% It is a closed convex surface in the wrench space that encloses the origin.
% combination of f and v, v is relative slip velocity
When the grasped object slips or is about to slip ($\twist \neq 0$), the friction wrench $\wrench$ lies on the limit surface.
Combining the LS with the maximal dissipation principle \cite{moreau.1973}, $\twist$ is normal to the limit surface at $\wrench$. %each friction wrench should be ideally on the surface of the LS, while its corresponding twist should be normal to the surface at this point.
This property can also be used to predict the twist $\predt$ with the surface normal of the LS for a given $\wrench$ acting on the body. 


% encloses origin
% convex

\subsection{Finding Wrench and Twist Pairs}
% sampling, normalization, downsampling etc
This section introduces the process to find the set of $P$ wrench and twist pairs $\W$ to fit the two limit surface models.

We first sample unit twists of the grasped object, defined in \sref{subsec:twist}, by sampling the triplet $\left(\linedir,\linepoint,h\right)$ and compute unit twists with $\normang=1$ using \eref{eq:twist} for each triplet. We also include the twists that are pure translations by using the unique samples of $\linedir$.
We then determine the friction wrench $\wrench$ for each unit twist with \eref{eq:frictionArea}.

Note that the twists for the fitting should be the relative twists between the grasped object and a gripper jaw. 
While the relative slip velocity can be computed with \eref{eq:projvp}, the relative angular velocity is not straightforward to determine. 
Therefore, we approximate the relative twist $\twistrel$ by using the sampled unit twist at the pressure center $\origin$, which can be considered as noisy sensory data.

We further normalize the wrench and twist pairs to fit the models for numerical stability. Denoting  $\wrench_\text{max} = [f_{x_\text{max}},f_{y_\text{max}},f_{z_\text{max}}, \tau_{x_\text{max}},\tau_{y_\text{max}},\tau_{z_\text{max}}]^T$ as the maximal magnitude of each dimension among all wrench samples, we normalize the $i$-th wrench ${\wrench}_i$ and twist $\twistreli$ by
\begin{equation}
	\normalwrench_i =  {\wrench}_i \oslash \wrench_\text{max}, \hspace{0.5em}
	\normaltwist_i = \frac{\twistreli \circ {\wrench_\text{max}}}{\norm{\twistreli \circ {\wrench_\text{max}}}}
\end{equation}
where $\oslash$ and $\circ$ are the Hadamard division and product, respectively. 
Note that $\normalwrench$ is dimensionless, $\normaltwist$ remains perpendicular to the LS at $\normalwrench$. 

% This section introduces the process to find the set of $P$ wrench and twist pairs $\W$ to fit the two limit surface models.

% We first sample unit twists of the grasped object, defined in \sref{subsec:twist}, by sampling the instantaneous screw axis $l$ and the scalar pitch $h$. 
% We then compute the friction wrench for each unit twist with \eref{eq:frictionArea}.
% Note that the twists for the fitting should be the relative twists between the grasped object and a gripper jaw. 
% While the relative slip velocity can be computed with \eref{eq:projvp}, the relative angular velocity is not straightforward to determine. 
% Therefore, we use the sampled unit twists for fitting, which can be considered as noisy sensory data.

% We further compute the normalized wrenches $\normalwrench$ and twists $\normaltwist$,  so that $\normalwrench$ is dimensionless, $\normaltwist$ remains perpendicular to the LS at $\normalwrench$. 
% We also downsample the pairs for computational efficiency. 
% Details about finding the pairs are in \aref{appendix:data} since its not our main contribution.

% We sample unit twists of the grasped object, defined in \ref{subsec:twist}, by sampling the instantaneous screw axis $l$ and the scalar pitch $h$. 
% We then compute the friction wrench for each unit twist with \eref{eq:frictionArea}.
% Note that the twists for the fitting should be the relative twists between the grasped object and a gripper jaw. 
% While the relative slip velocity can be computed with \eref{eq:projvp}, the relative angular velocity is not straightforward to determine. 
% Therefore, we use the sampled unit twists for fitting, which can be considered as noisy sensory data.

% We further compute the normalized wrenches $\normalwrench$ and twists $\normaltwist$,  so that $\normalwrench$ is dimensionless, $\normaltwist$ remains perpendicular to the LS at $\normalwrench$. 
We also downsample the pairs for computational efficiency. 
Details about sampling the triplets and reducing the number of pairs are in \aref{appendix:data}.

\subsection{Fitting an Ellipsoidal Model}
Given a set of normalized wrench and twist pairs $\W = \{ \normalwrench_{i\in \{ 1\ldotsc \nprs \}},\normaltwist_{i\in \{ 1\ldotsc \nprs \}} \}$, we formulate a convex optimization problem to fit a 6D ellipsoidal LS model. 

An arbitrarily oriented zero-centered 6D ellipsoid can be formulated as~\cite{chatterjee.1996}
\begin{equation}
\fe(\x,\Ae) = \x^T \Ae \x
\label{eq:ls_ellip}
\end{equation}
where $\Ae \in \mathbb{R}^{6 \times 6}$ is a symmetric positive-semidefinite matrix. 
The eigenvalues of $\Ae$ are the reciprocals of the squares of the semi-axes. 
The predicted twist $\predt \in \R{6}$ is normal to the ellipsoid at $\normalwrench$
\begin{equation}
\predt=\nabla \fe(\x,\Ae) = (\Ae + \Ae^T) \x =  2\Ae\x  
\label{eq:ls_ellip_gradient}
\end{equation}
Note that $\predt$ is not normalized, since a normalization leads to a non-convex optimization problem. 
Therefore, we introduce an additional variable $s_i \in \R{+}$ to scale $\normaltwist_i$, so that the magnitude of the twist does not affect the fitting error.

We denote $\errorwrenchi$ and $\errortwisti$ as the non-negative fitting error of $\normalwrench_i$ and $\normaltwist_i$, respectively.
$\errorwrenchi$ and $\errortwisti$ can be weighted with the non-negative variables $\weight_1$ and $\weight_2$, which are experimentally determined according to the reliability of the data. Fitting results with different weights are in \sref{xxx}.

We formulate the convex optimization problem to fit $\fe(\x,\Ae)=1$ by minimizing $\errorwrenchi$ and $\errortwisti$
\begin{equation}
\begin{aligned}
& \underset{\Ae,s_i,\errorwrenchi,\errortwisti}{\text{minimize}}
& &  \norm{\Ae}_F + \sum_{i=1}^\nprs(\weight_1 \bigcdot \errorwrenchi + \weight_2 \bigcdot  \errortwisti) \\
& \text{subject to}
& & \norm{\fe(\normalwrench_i,\Ae) - 1} \leq \errorwrenchi, \forall i \in  \{1 \ldotsc \nprs\} \\
%&&& \norm{(A^T + A)\boldw_i - \boldsymbol{s}_i \boldt_i} \leq \varepsilon_{\boldt_i}, \\
&&& \norm{\nabla \fe(\normalwrench_i,\Ae) - s_i \normaltwist_i} \leq \errortwisti, {s}_i \in \R{+} \\
&&& \Ae \succeq 0
\end{aligned}
\end{equation}
where $\norm{\Ae}_F$ is the Frobenius norm of $\Ae$ and regularizes the parameters. 

\subsection{Fitting a Quartic Model}
While an ellipsoid is a practical LS model for quasi-static~\cite{howe.1996} and sliding manipulation~\cite{howe.1996}, Zhou~et~al.~\cite{jiaji.2016} suggested that a convex quartic model better captures the force-motion relation for planar sliding. 
Therefore, we also generalize the 3D quartic model to 6D and fit the set $\W$ to the model. 

Denoting $\xnb_{j\in\{1\ldotsc 6\}}$ as the $j$-th dimension of a wrench sample $\normalwrench$, $d_j\in\mathbb{N}_0 = \{\mathbb{N} \cup \{0\}\}$ as the order where $\sum _{j=1}^6 d_j = 4$,  a six-variable quartic with $K$ monomials is 
\begin{equation}
\begin{aligned}
	&\fq(\x,\Aq)  = \sum _{k=1} ^K \left( a_k \prod_{j=1}^{6} \xnb_{j}^{d_j} \right), 
	\Aq = [a_1\ldotsc a_K]^T % &\sum _{j=1}^6 d_j = 4, \hspace{0.1em}  d_j \in \mathbb{N}_0 = \mathbb{N} \cup \{0\}.
\end{aligned}
\label{eq:ls_quartic}
\end{equation}
where $a_{k\in\{1 \ldotsc K\}} \in \mathbb{R}$ is the monomial coefficient. 
Here, $K = {4+6-1\choose6-1} = 126$. 
Note that we denote $\A$ as the LS model and $\Aq~\in~\R{126}$ for a quartic, whereas $\Ae~\in~\R{6\times 6}$ for an ellipsoid. %We use the same variable for consistency. 


\mysum{SOS-convex}
Zhou~et~al.~\cite{jiaji.2016} showed that it is essential to enforce the convexity of the quartic. 
However, the convexity is NP-hard to determine when the order is higher than two with more than one monomial. 
Magnani~et~al.~\cite{magnani.2005} proposed a relaxation technique by enforcing the convexity of $f_2$ only on a region by using the concept of sum-of-squares (SOS).
We use a similar technique to enforce the convexity.

We denote $\boldsymbol{z} \in \R{6}$ as a non-zero auxiliary variable, $\boldsymbol{y}(\x,\boldsymbol{z}) = [{\xnb_1  \boldsymbol{z}^T}, {\xnb_2 \boldsymbol{z}^T},  {\xnb_3 \boldsymbol{z}^T},  {\xnb_4 \boldsymbol{z}^T},  {\xnb_5 \boldsymbol{z}^T}, {\xnb_6 \boldsymbol{z}}^T]^T \in \mathbb{R}^{36}$. 
A polynomial $\fq(\x,\Aq)$ is defined as SOS convex, if there exists a positive-semidefinite matrix $\matr{Q} \in \R^{36 \times 36}$, so that the following equation holds
\begin{equation}
\boldsymbol{z}^T\nabla^2\fq(\x,\Aq)\boldsymbol{z}  = \boldsymbol{y}(\x,\boldsymbol{z})^T\matr{Q}\boldsymbol{y}(\x,\boldsymbol{z}).
\label{eq:sos_convex}
\end{equation}
We reformulate \eq~(\ref{eq:sos_convex}) as sparse linear constraints of $\Aq$ and the vectorization of $\matr{Q}$
\begin{equation}
	\matr{V}_1\mathrm{vec}(\matr{Q}) = \matr{V}_2\Aq
	\label{eq:sos_linear}
\end{equation} 
where $\matr{V}_1 \in \mathbb{N}_0^{441\times1296}$ and $\matr{V}_2\in \mathbb{N}_0^{441\times126}$ are constant sparse matrices and are essentially the number of each identical monomial on the left and right side of \eref{eq:sos_linear}, respectively.  %Here, there are 441 linear constraints since $\matr{V_1},\matr{V_2}$ are essentially the number of monomials and some monomials in \eref{eq:sos_convex} can be combined. 

%\begin{equation}
%	\mathrm{trace}(\matr{V_1}\matr{Q}) = \matr{V_2}\A,
%\end{equation}
%where $\matr{V_1} \in \mathbb{N}_0^{l\times36}$ and $\matr{V_2}\in \mathbb{N}_0^{l\times126}$ are constant sparse matrix.$N$ wrench and twist pairs with
We formulate the convex optimization problem to fit $\fq(\x,\Aq)=1$ also by minimizing $\errorwrenchi$ and $\errortwisti$
\begin{equation}
\begin{aligned}
& \underset{{\Aq,\matr{Q},s_i,\errorwrenchi,\errortwisti}}{\text{minimize}}
& &  \norm{\Aq} + \sum_{i=1}^\nprs(\weight_1 \bigcdot \errorwrenchi + \weight_2 \bigcdot  \errortwisti) \\
& \text{subject to}
& & \norm{\fq(\normalwrench_i,\Aq) - 1} \leq \errorwrenchi, \forall i \in  \{1 \ldotsc \nprs\}\\
&&& \norm{\nabla \fq(\normalwrench_i,\Aq) - s_i \normaltwist_i} \leq \errortwisti, {s}_i \in \R{+} \\
&&& 	\matr{V_1}\mathrm{vec}(\matr{Q}) = \matr{V_2}\Aq \\
&&& \matr{Q} \succeq 0.
\end{aligned}
\end{equation}

% With $\A$ being $\Ae$ and $\Aq$ for $\fe$ and $\fq$, respectively, the fitting error of $\nprs$ normalized wrenches $\normalwrench$ and twists $\normaltwist$ are

To evaluate the fitting results, we compute the fitting error for wrenches $\varepsilon_w$ with the mean distance of wrenches to the LS surface, while the twist fitting error $\varepsilon_t$ is the mean angle between the fitting and the predicted twist. With $f=\fe$ and $\A=\Ae$ for the ellipsoidal model, or $f=\fq$ and $\A=\Aq$ for the quartic, the fitting errors are %of $\nprs$ normalized wrenches $\normalwrench$ and twists $\normaltwist$ for both models $\fe,\fq$ are

\begin{equation}
\begin{aligned}
\varepsilon_w &= \frac{1}{\nprs}\sum_{i=1}^\nprs\errorwrenchi  \\
\varepsilon_t &= \frac{1}{\nprs}\sum_{i=1}^\nprs\cos^{-1}\left( \left(\frac{\nabla f(\normalwrench_i,\A)}{\nabla f(\normalwrench_i,\A)}\right)^T  \normaltwist_i\right)
\end{aligned}
\label{eq:fitting_error}
\end{equation}

With the 6DLS model for a non-planar surface contact, any friction wrench $\wrench$ of the contact is constrained to lie on or inside the LS
\begin{equation}
    f(\wrench,\A) \leq 1.
\label{eq:LS_constraint}
\end{equation}

% \begin{equation}
% \begin{aligned}
% \varepsilon_w &= \frac{1}{\nprs}\sum_{i=1}^\nprs\errorwrenchi  \\
% \varepsilon_t &= \frac{1}{\nprs}\sum_{i=1}^\nprs\cos^{-1}\left( \left(\frac{\nabla f_{\{
% e,q\}}(\normalwrench_i,\A_{\{
% e,q\}})}{\norm{\A\normalwrench_i}}\right)^T  \normaltwist_i\right)
% \end{aligned}
% \label{eq:fitting_error}
% \end{equation}
% where $\varepsilon_w$ indicates the mean distance of wrenches to the LS surface, $\varepsilon_t$ measures the mean angle between the predicted and the fitting twists. 






==> sections/old/9-multi-contacts-no-unit.tex <==


\mysum{Why need GWS in general}
%Fitting a 6DLS $\matr{A}$ requires on the contact profile including the surface geometry $\surface$ and the pressure distribution $\pressure$.
%Increasing the normal force $\boldsymbol{f}{_\perp}$ leads to an enlarged contact area until the maximum area is reached. 
%$\pressure$ then scales with the 
We introduce a 6DLS-based algorithm that predicts if a multi-contact grasp can resist a wrench disturbance by building a grasp wrench space. 
Each 6DLS and the GWS scale with the magnitude of the normal force $\norm{\fperp}$, if surface geometry $\surface$ and the shape of the pressure distribution remain constant.
This indicates changing $\norm{\fperp}$ leads to an unnecessary refitting of the 6DLS.
Therefore, the algorithm fits a unit 6DLS $\hat{\matr{A}}(\surface,\hat{\pressure})$ and builds the GWS by scaling $\hat{\matr{A}}$ with $\norm{\fperp}$, where $\int_{\surface} \hat{\pressure} = 1$.
Similar to the GWS construction process proposed by Farrari and Canny \cite{ferrari.1992}, the algorithm starts with linearly approximating the friction constraints of each contact for computational efficiency. 
%A grasp wrench space is commonly used to analyze the force and torque that a grasp can exert on an object and to predict the grasp success. 
%Given a fitted limit surface of each contact, we build the GWS by merging the wrenches of each contact into a single space, including the friction wrenches and the wrench impressed by the normal force,  defined as the normal wrench. 
%\mysum{applications of the GWS}
%Similar to the GWS construction for point contacts in~\cite{ferrari.1992} and for soft-finger contacts in  \cite{ciocarlie.2005}, we sample the LS surface to linearly approximate a fitted limit surface.

\subsection{Linearizing the limit surfaces}
Consider a grasp with $N$ contacts, denote $\matr{A}_i$ as the fitted 6DLS for the $i$-th contact with $i=1,\ldots,N$, $\boldsymbol{f}{_\perp}_i$ as the normal force, we compute the linearized friction constraints $\mathcal{F}_i$ by sampling the LS with $M$ vertices $\boldsymbol{x}_{i,j}$.
This indicates that any possible friction is bounded by the convex hull of $\boldsymbol{x}_{i,j}$:
%\begin{equation}
%\begin{aligned}
%	&\mathcal{F}_i = \{ \wrenchapprc_{i} | \wrenchapprc_{i} = \sum_{j=1}^{M} \alpha_{i,j} \cdot \boldsymbol{x}_{i,j} \wedge \\
%	& (\forall j: \alpha_{i,j} \geq 0) \wedge \sum_{j=1}^{M} \alpha_{i,j} = \norm{\boldsymbol{f}{_\perp}_i} \}
%\end{aligned}
%\end{equation}
\begin{equation}
\mathcal{F}_i =  \left\{ \sum_{j=1}^{M} \alpha_{i,j} \cdot \boldsymbol{x}_{i,j} \middle| (\forall j: \alpha_{i,j} \geq 0) \wedge \sum_{j=1}^{M} \alpha_{i,j} = \norm{\boldsymbol{f}{_\perp}_i} \right\} 
\end{equation}

We use naive approaches to obtain $\boldsymbol{x}_{i,j}$, where $\boldsymbol{x}_{i,j}$ are guaranteed to be on the surface, but may not be evenly distributed.

\subsubsection{Sampling the ellipsoidal model}
%After fitting the ellipsoidal limit surface model with Equation (\ref{eq:ls_ellip}), we obtain the fitted coefficient $\matr{A}$.
%We first compute  the semi-axes $r_m$  of the ellipsoid with $m=1,\ldots,6$.
We create $M$ random non-zero vectors $\tilde{\boldsymbol{x}}_j \in \mathbb{R}^{6}$. 
The surface point $\boldsymbol{x}_j$ is computed by $\boldsymbol{x}_j  =\tilde{\boldsymbol{x}}_j/d_j$, where $d_j = \sqrt{\sum_{m=1}^6 ({\tilde{x}_{j_m}^2}/{r_m^2}})$ is the distance between $\tilde{\boldsymbol{x}}_j$ to the ellipsoid origin, $r_m$ is the $m$-th semi-axis of the ellipsoid.
%For the $i$-th vector $\boldsymbol{x}_i$, we compute the corresponding point $\boldsymbol{y_i}$ on the surface of the ellipsoid with $\boldsymbol{y}_i  =\boldsymbol{x}_i/d_i$, where $d_i = \sqrt{\sum_{m=1}^6 ({x_{i_m}^2}/{r_m^2}})$ is the distance between $\boldsymbol{x}_i$ to the ellipsoid origin. 

%\begin{equation*}
%\boldsymbol{y}_i  = \frac{1}{d_i} \bigcdot \boldsymbol{x}_i \text{, where }
%d_i = \sqrt{\sum_{m=1}^6 \frac{x_{i_m}^2}{r_m^2}},
%\end{equation*}
%where $d_i$ is the distance of a sample $\boldsymbol{x}_i$ to the origin of the ellipsoid.

\subsubsection{Sampling the quartic model}
%The sampling strategy for an ellipsoid is not applicable for a quartic model since we can not obtain a sample on the surface based on the distance $d_i$. 
%Given $L$ random non-zero vectors $\tilde{\boldsymbol{x}}_l \in \mathbb{R}^{6}$ with $l=1,\ldots,L$ and $L>M$, we compute the value of $f_2(\tilde{\boldsymbol{x}},\matr{A})$ for each vector with \eq~(\ref{eq:ls_quartic}). %, where the fitted coefficients are summarized in $\matr{A}$.
%The surface vertices $\boldsymbol{x}_j$ are the subset of $\tilde{\boldsymbol{x}}$ that are on the isosurface $f_2(\tilde{\boldsymbol{x}},\matr{A}) = 1$.
Given $L$ random non-zero vectors $\tilde{\boldsymbol{x}}_l \in \mathbb{R}^{6}$ with $l=1,\ldots,L$ and $L>M$, the surface vertices $\boldsymbol{x}_j$ are the subset of $\tilde{\boldsymbol{x}}$ that are on the isosurface $f_2(\tilde{\boldsymbol{x}},\matr{A}) = 1$.


\subsection{Building the grasp wrench space}
We formulate the total wrench of the contact $\contactw_{i,j}$ by combining the friction constraints $\mathcal{F}_i$ and wrench impressed by $\boldsymbol{f}_{\perp_i}$:
\begin{equation}
\begin{aligned}
&\contactw_{i,j} = \begin{bmatrix} {\boldsymbol{f}_{\perp_i} + \fest_{i,j}} \\
{\boldsymbol{l}_{i}\times(\boldsymbol{f}_{\perp_i} + \fest_{i,j})+\tauest_{i,j}} \end{bmatrix}\text{, with } \tilde{\boldsymbol{w}}_{i,j} = \begin{bmatrix} {\fest_{i,j}} \\ {\tauest_{i,j}} \end{bmatrix} \\
& \boldsymbol{l}_{i} = \boldsymbol{\origin}_i - \boldsymbol{\origin}_{\text{GWS}},  \tilde{\boldsymbol{w}}_{i,j} \in  \mathcal{F}_i. 
\end{aligned}
\end{equation}
The center of mass of an object is typically selected as $\boldsymbol{\origin}_{\text{GWS}}$. 

Ferrari and Charry \cite{ferrari.1992} proposed two ways to build the GWS.
If the contact forces are independent, the GWS $\boldW_{L_\infty}$ is computed by:
\begin{equation}
\boldW_{L_\infty} = {Conv}(\oplus_{i=1}^N\{\contactw_{i,1},\ldots,\contactw_{i,j},\ldots,\contactw_{i,M}\}),
\end{equation}
where $Conv$ denotes the convex hull and $\oplus$ is the Minkowski sum operation. 
If the contact forces are not independent, the GWS $\boldW_{L_1}$ is computed by:
\begin{equation}
\boldW_{L_1} = {Conv}(\cup_{i=1}^N\{\contactw_{i,1},\ldots,\contactw_{i,j},\ldots,\contactw_{i,M}\}).
\end{equation}
We select $\boldW_{L_\infty}$ for experiments since Krug et al. \cite{krug2017grasp} suggested that $\boldW_{L_1}$ might be over-conservative. 

\subsection{Prediction}
Given a disturbance wrench $\disturbance \in \mathbb{R}^6$ and the GWS $\boldW_{L_\infty}$, the algorithm outputs a binary prediction $\hat{y} \in \{0,1\}$.
Denote $\hat{\boldsymbol{n}_k}$ as the outward normal of the $k$-th facet of $\boldW_{L_\infty}$, $\boldsymbol{a}_k \in \mathbb{R}^6$ as a point in the hyperplane of the facet, the prediction $\hat{y}=1$ if $\disturbance \in \boldW_{L_\infty}$:
\begin{equation}
	\left(  \forall k: \disturbance^T\hat{\boldsymbol{n}_k} < \boldsymbol{a}_k ^T\hat{\boldsymbol{n}_k} \rightarrow \hat{y}=1 \right) \wedge 	\left(\text{otherwise} \rightarrow \hat{y}=0 \right).
\end{equation}
Note that a fitted LS $\matr{A}_i$ depends on the contact surface $\surface$ and the pressure distribution $\pressure$.
!!! describe the motivation and the algorithm for $\hat{P}$ !!!

%After linearly approximating the fitted LS, we have $N$ friction wrenches of the $j$-th contact $\boldw_j =  [\boldsymbol{f}_j^T, \boldsymbol{\tau}_j^T]^T$ with respect to the friction center~$\boldsymbol{\origin}_j$. 
%Next, we compute the total wrench $\boldW_j$ of the contact $j$ with respect to the origin of the GWS $\boldsymbol{\origin}_{\text{GWS}}$ by combining $\boldw_j$ and the wrench caused by the normal force $\boldsymbol{f}{_\perp}_j$: 
%\begin{equation}
%\begin{aligned}
%&\boldW_j = \begin{bmatrix}{\boldsymbol{f}{_\perp}_j + \boldsymbol{f}_j}\\{\boldsymbol{l}_j\times(\boldsymbol{f}{_\perp}_j + \boldsymbol{f}_j)+\boldsymbol{\tau}_j} \end{bmatrix}\text{, with } \\
%& \boldsymbol{l}_j = \boldsymbol{\origin}_j - \boldsymbol{\origin}_{\text{GWS}}. 
%\end{aligned}
%\end{equation}
%The center of mass of an object is often selected as $\boldsymbol{\origin}_{\text{GWS}}$. 
%
%\mydo{explain why are they bounded}
%Ferrari and Charry \cite{ferrari.1992} proposed two ways to build the grasp wrench space of $M$ contacts.
%If the contact forces are independent, the GWS $\boldW_{L_\infty}$ is computed by:
%\begin{equation}
%	\boldW_{L_\infty} = ConvexHull(\oplus_{j=1}^M\{\boldW_{1},\ldots,\boldW_{j},\ldots,\boldW_{M}\}),
%\end{equation}
%where $\oplus$ is the Minkowski sum operation. 
%If the contact forces are not independent, the GWS $\boldW_{L_1}$ is computed by:
%\begin{equation}
%\boldW_{L_1} = ConvexHull(\cup_{j=1}^M\{\boldW_{1},\ldots,\boldW_{j},\ldots,\boldW_{M}\}).
%\end{equation}
%Here, the grasp success is inferred by checking if the GWS contains  the external disturbances.
%%We select the $\boldW_{L_1}$ in the physical experiments due to its computational efficiency. 
%Furthermore, the volume or the shortest vector of the GWS with a unit normal force is often used as a grasp quality metric~\cite{miller.2004,ciocarlie.2005,mahler.2017}. 
%



==> sections/old/9-multi-contacts-twist.tex <==
We introduce an algorithm to predict if a multi-contact grasp can resist the external wrench $\wext$, such as the  gravitational force and torque of the grasped object, given a 6DLS for each non-planar surface contact. We compute the grasp wrench space (GWS)~\cite{ferrari.1992}, or the space of wrenches that the contacts can apply to the object, to infer the grasp success. 
For the representative grasp in \fref{fig:headshot} with $\surface_1$ and $\surface_2$ being the contact surface between the cup and the left and right gripper jaw, respectively, the algorithm constructs the GWS given the limit surface models $\matr{A}_1$ for $\surface_1$ and $\matr{A}_2$ for $\surface_2$. %$\matr{A}_1$ and $\matr{A}_2$ are obtained by fit an ellipsoid or a quartic to normalized wrench and twist pairs introduced in \sref{sec:LS}.

This section starts with introducing the linearization technique for the limit surfaces and the construction of a grasp wrench space with these linearized friction constraints, followed by summarizing the algorithm to predict the grasp success.

\subsection{Linearizing the Limit Surface Models}
We linearly approximate the friction constraints of each contact for computational efficiency, similar to~\cite{ferrari.1992}. 
More specifically, instead of using \eref{eq:LS_constraint}, we constrain the friction wrench $\wrench$ to lie on or inside the discrete limit surfaces.

Given the 6DLS model $\A$, we discretize the limit surface by resampling $\A$ with $M$ vertices $\boldsymbol{x}_{m \in \{1\dots M\}} \in \R{6}$.
The friction wrench $\wrench$ can be approximated with a convex combination of the vertices $\wrench \approx \sum_{m=1}^M \alpha_m \boldsymbol{x}_m$, where $\alpha_m$ is the non-negative weight showing the contribution of $\boldsymbol{x}_m$ to $\wrench$. The set of friction constraints $\F$ is the convex hull of $\boldsymbol{x}_{m}$
\begin{equation}
\F =  \left\{ \sum_{m=1}^{M} \alpha_{m} \boldsymbol{x}_{m} \middle| (\forall m: \alpha_{m} \geq 0) \wedge \sum_{m=1}^{M} \alpha_{m} = 1 \right\}.
\end{equation}
Note that both $\boldsymbol{x}_{m}$ and $\F$ linearly scale with $\norm{\fperp}$.

We use different sampling approaches for the ellipsoid and the quartic to obtain $\boldsymbol{x}_m$, which are on the surface but may not be evenly sampled. 
Both approaches use $M$ randomly sampled non-zero vectors $\tilde{\boldsymbol{x}}_{m \in \{1\ldotsc M\}} \in \mathbb{R}^{6}$ to compute $\boldsymbol{x}_m$.
% We create $M$ non-zero vectors $\tilde{\boldsymbol{x}}_{i,j} \in \mathbb{R}^{6}$ sampled uniformly over $\left[-1, 1\right]$. 
\subsubsection{Sampling the ellipsoid}
We sample the ellipsoid surface described with $\Ae$ by first scaling  $\tilde{\boldsymbol{x}}_{m}$ then rotating it with the eigenvectors of $\Ae$ denoted as $\matr{X} \in \R{6\times 6}$, which defines the principle axes of the ellipsoid. 
Denoting $r_{j\in\{1\ldotsc 6\}}$ as the $j$-th semi-axis of the ellipsoid, the vertex $\boldsymbol{x}_m$ on the ellipsoid is
\begin{equation}
    \boldsymbol{x}_m  = \matr{X} \frac{\tilde{\boldsymbol{x}}_m}{\sqrt{\sum_{j=1}^6 ({\tilde{x}_{m_j}^2}/{r_j^2}})}.
\end{equation}


\subsubsection{Sampling the quartic}
The sampling strategy for an ellipsoid is not applicable for the quartic since the scaling factor can not be easily determined. 
To sample a quartic surface described with $\Aq$, we first define a ray that starts from the origin and goes through $\tilde{\boldsymbol{x}}_m$.
We parametrize the ray with $\lambda \bigcdot \tilde{\boldsymbol{x}}_m$, where $\lambda >0$ is a scaling factor.
The intersection point of the ray and the quartic surface is the vertex $\boldsymbol{x}_m$. We use the Newton's method to solve the equations for $\boldsymbol{x}_m$ and $\lambda$
\begin{equation}
    \fq(\boldsymbol{x}_m,\Aq) = 1 \text{ and }
    \boldsymbol{x}_m = \lambda \bigcdot \tilde{\boldsymbol{x}}_m.
\end{equation}




\subsection{Building the Grasp Wrench Space}
So far, the computed friction wrenches are for a single contact with respect to the local contact frame. 
We now consider the contact wrenches $\contactw_{m\in\{1 \ldotsc M\}}$, which is the combination of the resampled friction wrenches $\boldsymbol{x}_{m\in\{1 \ldotsc M\}}$ and the wrench impressed by the normal force $\fperp$.
We then express $\contactw_m$ for each contact of a grasp with respect to the object reference frame located at the center of mass $\origin_{\text{COM}}$ of the grasped object, and combine them into a single grasp wrench space. 
% We now express the wrenches of each contact with respect to a single reference frame located at the center of mass of the grasped object, and combine the wrenches of $N$ contacts of a grasp into a single grasp wrench space. 
% We now compute the total wrench that each contact can apply and combine the total wrenches of $N$ contacts of a grasp into a single grasp wrench space. 

Given the translation and rotation between the $n$-th contact and the object reference frame, denoted as $\boldsymbol{t}_n\in \R{3}$,$\matr{R}_n\in\R{3\times3}$ with $n=1 \ldotsc N$, respectively, the normal force $\fperp_{n}$, and the resampled wrenches on its LS $\boldsymbol{x}_{n,m}$, the contact wrench $\contactw_{n,m} \in \R{6}$ with respect to $\origin_{\text{COM}}$ is
\begin{equation}
\contactw_{n,m} = \begin{bmatrix} {\matr{R}_n & \boldsymbol{0}} \\
{\hat{\boldsymbol{t}}_n\matr{R}_n & \matr{R}_n} \end{bmatrix} \left(\boldsymbol{x}_{n,m} + \begin{bmatrix}{\fperp_n}\\{\boldsymbol{0}}\end{bmatrix}\right)
\end{equation}
where $\hat{\boldsymbol{t}}_n \in \R{3\times3}$ is the cross product matrix of $\boldsymbol{t}_n$.
% For the $n$-th contact, given the normal force $\fperp_{n\in\{1 \ldotsc N\}}$, the pressure center $\origin_n$, and the resampled wrenches on its LS $\boldsymbol{x}_{n,m \in \{1\ldotsc M\}}$, we compute the total wrench $\contactw_{n,m}$ with respect to the center of mass $\origin_{\text{COM}}$ of the grasped object. By writing $\boldsymbol{x}_{n,m} = [ \boldsymbol{f}_{n,m}^T , \boldsymbol{\tau}_{n,m}^T ]^T$, the total wrench, consists of the friction wrench and the wrench impressed by $\fperp_n$, is 
% \begin{equation}
% \contactw_{n,m} = \begin{bmatrix} {\fperp_n + \boldsymbol{f}_{n,m}} \\
% {(\origin_n - \origin_\text{COM})\times(\fperp_n + \boldsymbol{f}_{n,m})+\boldsymbol{\tau}_{n,m}} \end{bmatrix}.
% \end{equation}


Ferrari and Canny~\cite{ferrari.1992} proposed two ways to build the GWS: by upper bounding the magnitude of each contact force individually or by bounding the sum magnitude of the contact normal forces. 
We select the former since Krug~et~al. \cite{krug2017grasp} suggested that the latter is over-conservative. 
The grasp wrench space $\boldW$ is
\begin{equation}
\boldW = \text{Conv}(\oplus_{n=1}^N\{\contactw_{n,1} \ldotsc \contactw_{n,m} \ldotsc \contactw_{n,M}\})
\end{equation}
where Conv$(\bigcdot)$ denotes the convex hull and $\oplus$ is the Minkowski sum operation. 
% If the contact forces are independent, the GWS $\boldW_{L_\infty}$ is computed by:
% \begin{equation}
% \boldW_{L_\infty} = {Conv}(\oplus_{i=1}^N\{\contactw_{i,1},\ldotsc,\contactw_{i,j},\ldotsc,\contactw_{i,M}\}),
% \end{equation}
% where $Conv$ denotes the convex hull and $\oplus$ is the Minkowski sum operation. 
% If the contact forces are not independent, the GWS $\boldW_{L_1}$ is computed by:
% \begin{equation}
% \boldW_{L_1} = {Conv}(\cup_{i=1}^N\{\contactw_{i,1},\ldotsc,\contactw_{i,j},\ldotsc,\contactw_{i,M}\}).
% \end{equation}
% We select $\boldW_{L_\infty}$ for experiments since Krug et al. \cite{krug2017grasp} suggested that $\boldW_{L_1}$ is over-conservative. 

\subsection{Prediction}
% Based on the grasp wrench space $\boldW$, 
The algorithm now predicts if the grasp can resist the external wrench $\wext \in \mathbb{R}^6$ by checking if the opposite wrench $-\wext$ is on or inside the grasp wrench space $\boldW$.

Given $\boldW$ with $L$ facets, denoting $\hat{\boldsymbol{n}}_{r\in \{1 \ldotsc L\}} \in \R{6}$ as the outward normal of the $r$-th facet of $\boldW$, $\boldsymbol{a}_r \in \R{6}$ as a point in the hyperplane of the facet, the binary prediction ${y} \in \{0,1\}$ is 
\begin{equation}
y = 
\begin{dcases*}
	1 & if $-\wext^T\hat{\boldsymbol{n}}_r \leq \boldsymbol{a}_r ^T\hat{\boldsymbol{n}}_r, \forall r \in \{1 \ldotsc L\}$ \\
	0 & otherwise.
\end{dcases*}
\end{equation}


% \begin{equation}
% 	\left(  \forall k: (-\wext)^T\hat{\boldsymbol{n}}_k < \boldsymbol{a}_k ^T\hat{\boldsymbol{n}}_k \rightarrow {y}=1 \right) \wedge 	\left(\text{otherwise} \rightarrow {y}=0 \right).
% \end{equation}

\subsection{Algorithm}
We summarize the algorithm to predict multi-contact grasp success given the contact surface $\surface$ and the pressure distribution $\pressure$ of each contact. 

Note that the limit surface of each contact linearly scales with the magnitude of the normal force $\norm{\fperp}$ of the contact, if $\surface$ and the shape of the pressure distribution remain constant.
This indicates that changing $\norm{\fperp}$ leads to an unnecessary fitting of the 6DLS.
Therefore, we compute wrench and twist pairs for $\surface$ with a unit pressure distribution $\hat{\pressure}$ with $\int_{\surface} \hat{\pressure} =\int_{\surface} {\pressure}/\norm{\fperp}= 1$, then fits the 6DLS $\ASP$ to the pairs and stores it in the dataset $\D$ for reuses.
Algorithm~\ref{algo:6dls_predict} summarizes the process to predict grasp success.

\input{algos/algo-exp-ls}



%After linearly approximating the fitted LS, we have $N$ friction wrenches of the $j$-th contact $\boldw_j =  [\boldsymbol{f}_j^T, \boldsymbol{\tau}_j^T]^T$ with respect to the friction center~$\boldsymbol{\origin}_j$. 
%Next, we compute the total wrench $\boldW_j$ of the contact $j$ with respect to the origin of the GWS $\boldsymbol{\origin}_{\text{GWS}}$ by combining $\boldw_j$ and the wrench caused by the normal force $\boldsymbol{f}{_\perp}_j$: 
%\begin{equation}
%\begin{aligned}
%&\boldW_j = \begin{bmatrix}{\boldsymbol{f}{_\perp}_j + \boldsymbol{f}_j}\\{\boldsymbol{l}_j\times(\boldsymbol{f}{_\perp}_j + \boldsymbol{f}_j)+\boldsymbol{\tau}_j} \end{bmatrix}\text{, with } \\
%& \boldsymbol{l}_j = \boldsymbol{\origin}_j - \boldsymbol{\origin}_{\text{GWS}}. 
%\end{aligned}
%\end{equation}
%The center of mass of an object is often selected as $\boldsymbol{\origin}_{\text{GWS}}$. 
%
%\mydo{explain why are they bounded}
%Ferrari and Charry \cite{ferrari.1992} proposed two ways to build the grasp wrench space of $M$ contacts.
%If the contact forces are independent, the GWS $\boldW_{L_\infty}$ is computed by:
%\begin{equation}
%	\boldW_{L_\infty} = ConvexHull(\oplus_{j=1}^M\{\boldW_{1},\ldotsc,\boldW_{j},\ldotsc,\boldW_{M}\}),
%\end{equation}
%where $\oplus$ is the Minkowski sum operation. 
%If the contact forces are not independent, the GWS $\boldW_{L_1}$ is computed by:
%\begin{equation}
%\boldW_{L_1} = ConvexHull(\cup_{j=1}^M\{\boldW_{1},\ldotsc,\boldW_{j},\ldotsc,\boldW_{M}\}).
%\end{equation}
%Here, the grasp success is inferred by checking if the GWS contains  the external disturbances.
%%We select the $\boldW_{L_1}$ in the physical experiments due to its computational efficiency. 
%Furthermore, the volume or the shortest vector of the GWS with a unit normal force is often used as a grasp quality metric~\cite{miller.2004,ciocarlie.2005,mahler.2017}. 
%



==> sections/old/9-multi-contacts-unit.tex <==
We introduce an algorithm to predict if a multi-contact grasp can resist the external wrench $\wext$, such as the  gravitational force and torque of the grasped object, given a 6DLS for each non-planar surface contact. We compute the grasp wrench space (GWS) \cite{ferrari.1992}, or the space of wrenches that the contacts can apply to the object, to infer the grasp success. 
For the representative grasp in \fref{fig:headshot} with $\surface_1$ and $\surface_2$ being the contact surface between the cup and the left and right gripper jaw, respectively, the algorithm constructs the GWS given the limit surface models $\matr{A}_1$ for $\surface_1$ and $\matr{A}_2$ for $\surface_2$. %$\matr{A}_1$ and $\matr{A}_2$ are obtained by fit an ellipsoid or a quartic to normalized wrench and twist pairs introduced in \sref{sec:LS}.

We start with linearizing the limit surface to build a grasp wrench space, followed by summarizing the algorithm to predict the grasp success.

\subsection{Linearizing the limit surfaces}
Similar to the GWS construction process proposed by Ferrari and Canny \cite{ferrari.1992}, the algorithm starts with linearly approximating the friction constraints of each contact for computational efficiency. 

Given a 6DLS $\ASPi$ for the $i$-th contact with $i=1,\ldots,N$, we compute the linearized friction constraints $\hat{\mathcal{F}}_i$ by sampling the LS with vertices $\boldsymbol{x}_{i,j} \in \mathbb{R}^6, j=1,\ldots,M$.
This indicates that any possible friction is upper bounded by the convex hull of $\boldsymbol{x}_{i,j}$:

\begin{equation}
\hat{\mathcal{F}}_i =  \left\{ \sum_{j=1}^{M} \alpha_{i,j} \cdot \boldsymbol{x}_{i,j} \middle| (\forall j: \alpha_{i,j} \geq 0) \wedge \sum_{j=1}^{M} \alpha_{i,j} = 1 \right\} 
\end{equation}

We use naive sampling approaches for $\boldsymbol{x}_{i,j}$ that may not be evenly distributed.

\subsubsection{Sampling the ellipsoidal model}
We create $M$ non-zero vectors $\tilde{\boldsymbol{x}}_{i,j} \in \mathbb{R}^{6}$ sampled uniformly over $\left[-1, 1\right]$. 
Denoting $d_{i,j} = \sqrt{\sum_{m=1}^6 ({\tilde{x}_{{i,j}_m}^2}/{r_m^2}})$ as the distance between $\tilde{\boldsymbol{x}}_{i,j}$ to the ellipsoid origin, where $r_m$ is the $m$-th semi-axis of the ellipsoid, the surface point $\boldsymbol{x}_{i,j}$ is computed by $\boldsymbol{x}_{i,j}  =\tilde{\boldsymbol{x}}_{i,j}/d_{i,j}$.

\subsubsection{Sampling the quartic model}
%The sampling strategy for an ellipsoid is not applicable for a quartic model since we can not obtain a sample on the surface based on the distance $d_i$. 
%Given $L$ random non-zero vectors $\tilde{\boldsymbol{x}}_l \in \mathbb{R}^{6}$ with $l=1,\ldots,L$ and $L>M$, we compute the value of $f_2(\tilde{\boldsymbol{x}},\matr{A})$ for each vector with \eq~(\ref{eq:ls_quartic}). %, where the fitted coefficients are summarized in $\matr{A}$.
%The surface vertices $\boldsymbol{x}_j$ are the subset of $\tilde{\boldsymbol{x}}$ that are on the isosurface $f_2(\tilde{\boldsymbol{x}},\matr{A}) = 1$.
Given $L$ uniformly sampled random non-zero vectors $\tilde{\boldsymbol{x}}_{i,l} \in \mathbb{R}^{6}$ over  $\left[-1, 1\right]$  with $l=1,\ldots,L$ and $L>M$, the surface vertices $\boldsymbol{x}_{i,j}$ are the subset of the vectors that are close to the isosurface:  $\norm{f_2(\tilde{\boldsymbol{x}}_{i,l},\matr{A}_i) - 1} \leq \epsilon$ computed with \eq~(\ref{eq:ls_quartic}).
We select $\epsilon=0.01$ for physical experiments. 


\subsection{Building the grasp wrench space}
We formulate the total unit wrench $\contactwunit_{i,j}$ in the object frame by combining the linearized friction constraints  $\hat{\mathcal{F}}_i$ and the wrench impressed by $\fperpiunit$:
\begin{equation}
\contactwunit_{i,j} = \begin{bmatrix} {\fperpiunit + \fest_{i,j}} \\
{\boldsymbol{l}_{i}\times(\fperpiunit + \fest_{i,j})+\tauest_{i,j}} \end{bmatrix}, \hat{\boldsymbol{w}}_{i,j} = \begin{bmatrix} {\fest_{i,j}} \\ {\tauest_{i,j}}  \end{bmatrix} \in  \hat{\mathcal{F}}_i,
\end{equation}
with the torque arm being $\boldsymbol{l}_{i} = \boldsymbol{\origin}_{c_i} - \boldsymbol{\origin}_\boldW$, where $\boldsymbol{\origin}_{c_i} $ is the contact location in the object frame and $\boldsymbol{\origin}_\boldW$ is the center of mass (COM) of an object. 
The total wrench of the $i$-th contact is computed by $\contactw_{i,j} = \norm{\fperp_i} \cdot \contactwunit_{i,j}$

Ferrari and Canny \cite{ferrari.1992} proposed two ways to build the GWS.
If the contact forces are independent, the GWS $\boldW_{L_\infty}$ is computed by:
\begin{equation}
\boldW_{L_\infty} = {Conv}(\oplus_{i=1}^N\{\contactw_{i,1},\ldots,\contactw_{i,j},\ldots,\contactw_{i,M}\}),
\end{equation}
where $Conv$ denotes the convex hull and $\oplus$ is the Minkowski sum operation. 
If the contact forces are not independent, the GWS $\boldW_{L_1}$ is computed by:
\begin{equation}
\boldW_{L_1} = {Conv}(\cup_{i=1}^N\{\contactw_{i,1},\ldots,\contactw_{i,j},\ldots,\contactw_{i,M}\}).
\end{equation}
We select $\boldW_{L_\infty}$ for experiments since Krug et al. \cite{krug2017grasp} suggested that $\boldW_{L_1}$ is over-conservative. 

\subsection{Prediction}


Based on a disturbance wrench $\disturbance \in \mathbb{R}^6$ and the GWS $\boldW_{L_\infty}$, the algorithm computes a binary prediction ${y} \in \{0,1\}$.

Each 6DLS linearly scales with the magnitude of the normal force $\norm{\fperp}$ of the contact, if $\surface$ and the shape of the pressure distribution remain constant.
This indicates that changing $\norm{\fperp}$ leads to an unnecessary fitting of the 6DLS.
Therefore, the algorithm computes wrench and twist pairs for $\surface$ with a unit pressure distribution $\hat{\pressure}$ with $\int_{\surface} \hat{\pressure} =\int_{\surface} {\pressure}/\norm{\fperp}= 1$, then fits the 6DLS $\ASP$ to the pairs and stores it in a dataset for reuses.


Denoting $\hat{\boldsymbol{n}}_k$ as the outward normal of the $k$-th facet of $\boldW_{L_\infty}$, $\boldsymbol{a}_k \in \mathbb{R}^6$ as a point in the hyperplane of the facet, the prediction ${y}=1$, if $\disturbance \in \boldW_{L_\infty}$:
\begin{equation}
	\left(  \forall k: \disturbance^T\hat{\boldsymbol{n}}_k < \boldsymbol{a}_k ^T\hat{\boldsymbol{n}}_k \rightarrow {y}=1 \right) \wedge 	\left(\text{otherwise} \rightarrow {y}=0 \right).
\end{equation}

Algorithm~\ref{algo:6dls_predict} summarizes the process to predict grasp success.

\input{algos/algo-exp-ls}



%After linearly approximating the fitted LS, we have $N$ friction wrenches of the $j$-th contact $\boldw_j =  [\boldsymbol{f}_j^T, \boldsymbol{\tau}_j^T]^T$ with respect to the friction center~$\boldsymbol{\origin}_j$. 
%Next, we compute the total wrench $\boldW_j$ of the contact $j$ with respect to the origin of the GWS $\boldsymbol{\origin}_{\text{GWS}}$ by combining $\boldw_j$ and the wrench caused by the normal force $\boldsymbol{f}{_\perp}_j$: 
%\begin{equation}
%\begin{aligned}
%&\boldW_j = \begin{bmatrix}{\boldsymbol{f}{_\perp}_j + \boldsymbol{f}_j}\\{\boldsymbol{l}_j\times(\boldsymbol{f}{_\perp}_j + \boldsymbol{f}_j)+\boldsymbol{\tau}_j} \end{bmatrix}\text{, with } \\
%& \boldsymbol{l}_j = \boldsymbol{\origin}_j - \boldsymbol{\origin}_{\text{GWS}}. 
%\end{aligned}
%\end{equation}
%The center of mass of an object is often selected as $\boldsymbol{\origin}_{\text{GWS}}$. 
%
%\mydo{explain why are they bounded}
%Ferrari and Charry \cite{ferrari.1992} proposed two ways to build the grasp wrench space of $M$ contacts.
%If the contact forces are independent, the GWS $\boldW_{L_\infty}$ is computed by:
%\begin{equation}
%	\boldW_{L_\infty} = ConvexHull(\oplus_{j=1}^M\{\boldW_{1},\ldots,\boldW_{j},\ldots,\boldW_{M}\}),
%\end{equation}
%where $\oplus$ is the Minkowski sum operation. 
%If the contact forces are not independent, the GWS $\boldW_{L_1}$ is computed by:
%\begin{equation}
%\boldW_{L_1} = ConvexHull(\cup_{j=1}^M\{\boldW_{1},\ldots,\boldW_{j},\ldots,\boldW_{M}\}).
%\end{equation}
%Here, the grasp success is inferred by checking if the GWS contains  the external disturbances.
%%We select the $\boldW_{L_1}$ in the physical experiments due to its computational efficiency. 
%Furthermore, the volume or the shortest vector of the GWS with a unit normal force is often used as a grasp quality metric~\cite{miller.2004,ciocarlie.2005,mahler.2017}. 
%



==> sections/old/9-multi-contacts_old.tex <==


\mysum{Why need GWS in general}

%The presented limit surface models describe a single surface contact. 
Multiple contacts may occur when grasping an object. 
A grasp wrench space is commonly used to analyze the force and torque that a grasp can exert on an object and to predict the grasp success. 
Given a fitted limit surface of each contact, we build the GWS by merging the wrenches of each contact into a single space, including the friction wrenches and the wrench impressed by the normal force,  defined as the normal wrench. 
%The limit surfaces of multiple contacts are typically combined into a single space, defined as the grasp wrench space.
\mysum{applications of the GWS}
%The GWS is widely used for grasp stability assessment \cite{krug.2016} and as a grasp quality metric \cite{ferrari.1992,miller.2004,ciocarlie.2005}, since it estimates the maximal friction wrench of a grasp and hence the amount of disturbances that the grasp can balance.
%The GWS is built by merging the wrenches of each contact into a single space, including the friction wrenches and the wrench impressed by the normal force,  defined as the normal wrench. 
Similar to the GWS construction for point contacts in~\cite{ferrari.1992} and for soft-finger contacts in  \cite{ciocarlie.2005}, we sample the LS surface to linearly approximate a fitted limit surface.

%The sampling strategies for the ellipsoidal and the quartic polynomial model are introduced in the following. 
%The GWS is used for stability prediction in Section~\ref{subsec:roboExp}.

\mydo{Maybe put sampling the LS into experiments}

\subsection{Sampling the limit surfaces}
We use naive approaches to sample the surfaces, where the points are guaranteed to be on the surface, but may not be evenly sampled and may not contain the extrema of each variable.
\subsubsection{Sampling the ellipsoidal model}
%After fitting the ellipsoidal limit surface model with Equation (\ref{eq:ls_ellip}), we obtain the fitted coefficient $\matr{A}$.
We first compute  the semi-axes $r_m$  of a fitted ellipsoid $\matr{A}$, given the eigenvalues of $\matr{A}$ are $r_m^{-2}$ with $m=1,\ldots,6$.
We generate $N$ random non-zero vectors $\boldsymbol{x}^{6 \times N}$. 
For the  $i$-th vector $\boldsymbol{x}_i$, we compute the corresponding point $\boldsymbol{y_i}$ on the surface of the ellipsoid with $\boldsymbol{y}_i  =\boldsymbol{x}_i/d_i$, where $d_i = \sqrt{\sum_{m=1}^6 ({x_{i_m}^2}/{r_m^2}})$ is the distance between $\boldsymbol{x}_i$ to the ellipsoid origin. 

%\begin{equation*}
%\boldsymbol{y}_i  = \frac{1}{d_i} \bigcdot \boldsymbol{x}_i \text{, where }
%d_i = \sqrt{\sum_{m=1}^6 \frac{x_{i_m}^2}{r_m^2}},
%\end{equation*}
%where $d_i$ is the distance of a sample $\boldsymbol{x}_i$ to the origin of the ellipsoid.

\subsubsection{Sampling the quartic model}
%The sampling strategy for an ellipsoid is not applicable for a quartic model since we can not obtain a sample on the surface based on the distance $d_i$. 
Given $\matr{A}$ of a fitted quartic, we generate $N$ random vectors $\boldsymbol{x}^{6 \times N}$ and compute the value of $f_2(\boldsymbol{x},\matr{A})$ for each vector with \eq~(\ref{eq:ls_quartic}). %, where the fitted coefficients are summarized in $\matr{A}$.
The samples on the surface  $\boldsymbol{y}$ are the subset of $\boldsymbol{x}$ that are on the isosurface $f_2(\boldsymbol{x},\matr{A}) = 1$.

\subsection{Building the grasp wrench space}
After linearly approximating the fitted LS, we have $N$ friction wrenches of the $j$-th contact $\boldw_j =  [\boldsymbol{f}_j^T, \boldsymbol{\tau}_j^T]^T$ with respect to the friction center~$\boldsymbol{\origin}_j$. 
Next, we compute the total wrench $\boldW_j$ of the contact $j$ with respect to the origin of the GWS $\boldsymbol{\origin}_{\text{GWS}}$ by combining $\boldw_j$ and the wrench caused by the normal force $\boldsymbol{f}{_\perp}_j$: 
\begin{equation}
\begin{aligned}
&\boldW_j = \begin{bmatrix}{\boldsymbol{f}{_\perp}_j + \boldsymbol{f}_j}\\{\boldsymbol{l}_j\times(\boldsymbol{f}{_\perp}_j + \boldsymbol{f}_j)+\boldsymbol{\tau}_j} \end{bmatrix}\text{, with } \\
& \boldsymbol{l}_j = \boldsymbol{\origin}_j - \boldsymbol{\origin}_{\text{GWS}}. 
\end{aligned}
\end{equation}
The center of mass of an object is often selected as $\boldsymbol{\origin}_{\text{GWS}}$. 

\mydo{explain why are they bounded}
Ferrari and Charry \cite{ferrari.1992} proposed two ways to build the grasp wrench space of $M$ contacts.
If the contact forces are independent, the GWS $\boldW_{L_\infty}$ is computed by:
\begin{equation}
	\boldW_{L_\infty} = ConvexHull(\oplus_{j=1}^M\{\boldW_{1},\ldots,\boldW_{j},\ldots,\boldW_{M}\}),
\end{equation}
where $\oplus$ is the Minkowski sum operation. 
If the contact forces are not independent, the GWS $\boldW_{L_1}$ is computed by:
\begin{equation}
\boldW_{L_1} = ConvexHull(\cup_{j=1}^M\{\boldW_{1},\ldots,\boldW_{j},\ldots,\boldW_{M}\}).
\end{equation}
Here, the grasp success is inferred by checking if the GWS contains  the external disturbances.
%We select the $\boldW_{L_1}$ in the physical experiments due to its computational efficiency. 
Furthermore, the volume or the shortest vector of the GWS with a unit normal force is often used as a grasp quality metric~\cite{miller.2004,ciocarlie.2005,mahler.2017}. 




==> tabs/tableDiscretizationEffect.tex <==
\begin{table}
	\begin{center}
		\caption{Discretization effect on the friction wrench error}
		
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
			\hline
			\multirow{3}{*}{ID}	 & \multicolumn{8}{c|}{Error of maximal wrench with different sizes of elements (\%)} \\\cline{2-9}			
			 & \multicolumn{8}{c|}{Uniform pressure distribution} \\\cline{2-9}
			
			  & 0.6 & 0.5 & 0.4 &  0.3 & 0.2 & 0.1 & 0.03 & 0.01\\ \hline
			
			 S1 & 5.12 & 3.85 & 2.08 & 1.43 & 0.58 & 0.15 & 0.01 & 0.00  \\\hline
			
			 S2 & 7.43 & 5.62 & 3.30 & 1.82 & 0.80 & 0.20 & 0.02 & 0.00 \\\hline
			 S3  & 14.05 & 10.05 & 6.23 & 3.52 & 1.65 & 0.51 & 0.07 & 0.01 \\\hline
			 S4  & 27.27 & 17.17 & 12.09 & 8.41 & 3.56 & 1.07 & 0.16 & 0.03 \\ \hline
			 S5  & 17.12 & 9.50 & 5.99 & 3.66 & 1.63 & 0.42 & 0.06 & 0.01 \\ \hline
			 S6  & 16.58 & 10.70 & 6.86 & 4.04 & 1.63 & 0.75 & 0.17 & 0.06 \\
			  \hline
			 \textbf{m}  & \textbf{14.60}  &  \textbf{9.48}  &  \textbf{6.09}  &  \textbf{3.81}   & \textbf{1.64}  &  \textbf{0.52}  &  \textbf{0.08} &   \textbf{0.02} \\ 		
			
			\hline
			\hline
			 & \multicolumn{8}{c|}{Hetztian pressure distribution} \\\hline
			 S1  & 4.83 & 3.81 & 2.20 & 1.72 & 0.97 & 0.61 & 0.51 & 0.50 
			  \\ \hline
			
			 S2 & 6.81 & 5.17 & 3.16 & 1.90 & 1.00 & 0.51 & 0.41 & 0.39 
			 \\ \hline
			 S3 & 13.54 & 9.62 & 6.02 & 3.45 & 1.73 & 0.66 & 0.37 & 0.32 
			  \\ \hline
			 S4 &26.92 & 16.95 & 11.87 & 8.30 & 3.53 & 1.08 & 0.35 & 0.16 
			  \\ \hline
			 S5 &16.40 & 9.15 & 5.63 & 3.47 & 1.49 & 0.33 & 0.08 & 0.09 
			  \\ \hline
			 S6 & 16.24 & 10.45 & 6.93 & 4.11 & 1.67 & 0.87 & 0.43 & 0.26 
			 \\ 
			  \hline
			 \textbf{m}  & \textbf{14.12}  &  \textbf{9.19}  &  \textbf{5.97}  &  \textbf{3.83}   & \textbf{1.73}  &  \textbf{0.68}  &  \textbf{0.36} &   \textbf{0.29} \\ 
			\hline
			\hline
			\multirow{2}{*}{}	 & \multicolumn{8}{c|}{Error of surface area with different sizes of elements (\%)} \\\hline
			
			
			
			S1  & 0.64 & 0.51 & 0.29 & 0.18 & 0.08 & 0.02 & 0.00 & 0.00  \\ \hline
			
			 S2  & 1.13 & 0.84 & 0.51 & 0.29 & 0.13 & 0.03 & 0.00 & 0.00 \\ \hline
			 S3  &7.20 & 5.20 & 3.12 & 1.77 & 0.80 & 0.22 & 0.02 & 0.00 \\ \hline
			 S4  & 15.84 & 9.76 & 6.65 & 4.55 & 1.83 & 0.69 & 0.07 & 0.02 \\ \hline
			 S5  & 7.22 & 4.16 & 2.64 & 1.75 & 0.79 & 0.21 & 0.02 & 0.00\\ \hline
			 S6  & 15.24 & 9.54 & 8.02 & 5.11 & 2.31 & 1.02 & 0.16 & 0.05 \\ \hline
			 \textbf{m}  & 1\textbf{7.88}  &  \textbf{5.00}  &  \textbf{3.54}  &  \textbf{2.28}   & \textbf{0.99}  &  \textbf{0.36}  &  \textbf{0.05} &   \textbf{0.01} \\ 
			
			\hline
		\end{tabular}
	\end{center}
\end{table}

%%%%%%%%%%% Two digits %%%%%%%%%%%%%
%\begin{table}
%	\begin{center}
%		\caption{Discretization effect on the friction wrench error}
%		
%		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
%			\hline
%			
%			\multirow{3}{*}{P} & \multirow{3}{*}{ID}	 & \multicolumn{8}{c|}{Error of maximal wrench with different sizes of elements (\%)} \\\cline{3-10}
%			
%			&  & 0.6 & 0.5 & 0.4 &  0.3 & 0.2 & 0.1 & 0.03 & 0.01\\ \hline
%	
%			\multirow{6}{*}{U} & S1 & 5.12 & 3.85 & 2.08 & 1.43 & 0.58 & 0.15 & 0.01 & 0.00  \\ \cline{2-10}
%				
%			& S2 & 7.43 & 5.62 & 3.30 & 1.82 & 0.80 & 0.20 & 0.02 & 0.00 \\ \cline{2-10}
%			& S3  & 14.05 & 10.05 & 6.23 & 3.52 & 1.65 & 0.51 & 0.07 & 0.01 \\ \cline{2-10}
%			& S4  & 27.27 & 17.17 & 12.09 & 8.41 & 3.56 & 1.07 & 0.16 & 0.03 \\ \cline{2-10}
%			& S5  & 17.12 & 9.50 & 5.99 & 3.66 & 1.63 & 0.42 & 0.06 & 0.01 \\ \cline{2-10}
%			& S6  & 16.58 & 10.70 & 6.86 & 4.04 & 1.63 & 0.75 & 0.17 & 0.06 \\ \cline{2-10}
%
%
%			\hline
%			\hline
%			\multirow{6}{*}{H} & S1  & 23.31 & 19.48 & 14.12 & 12.01 & 8.71 & 6.17 & 4.66 & 4.27 \\ \cline{2-10}
%			
%			& S2 & 30.41 & 25.37 & 19.63 & 15.50 & 11.76 & 8.81 & 7.14 & 6.70\\ \cline{2-10}
%			& S3 & 15.49 & 12.12 & 9.17 & 6.79 & 4.95 & 3.38 & 2.36 & 2.04 \\ \cline{2-10}
%			& S4 & 28.42 & 19.43 & 12.98 & 9.53 & 4.49 & 1.73 & 1.02 & 0.95\\ \cline{2-10}
%			& S5 & 24.13 & 15.40 & 9.83 & 7.06 & 3.69 & 1.52 & 0.59 & 0.41\\ \cline{2-10}
%			& S6 &26.07 & 15.71 & 9.07 & 5.90 & 2.89 & 0.83 & 0.50 & 0.39\\ \cline{2-10}	
%			\hline
%			\hline
%			\multirow{3}{*}{} & \multirow{3}{*}{}	 & \multicolumn{8}{c|}{Error of surface area with different sizes of elements (\%)} \\\cline{2-10}
%			
%
%			
%			\multirow{6}{*}{U/H} & S1  & 0.64 & 0.51 & 0.29 & 0.18 & 0.08 & 0.02 & 0.00 & 0.00  \\ \cline{2-10}
%			
%			& S2  & 1.13 & 0.84 & 0.51 & 0.29 & 0.13 & 0.03 & 0.00 & 0.00 \\ \cline{2-10}
%			& S3  &7.20 & 5.20 & 3.12 & 1.77 & 0.80 & 0.22 & 0.02 & 0.00 \\ \cline{2-10}
%			& S4  & 15.84 & 9.76 & 6.65 & 4.55 & 1.83 & 0.69 & 0.07 & 0.02 \\ \cline{2-10}
%			& S5  & 7.22 & 4.16 & 2.64 & 1.75 & 0.79 & 0.21 & 0.02 & 0.00\\ \cline{2-10}
%			& S6  & 15.24 & 9.54 & 8.02 & 5.11 & 2.31 & 1.02 & 0.16 & 0.05 \\ \cline{2-10}
%			
%			\hline
%		\end{tabular}
%	\end{center}
%\end{table}


%\begin{table}
%	\begin{center}
%	\caption{Discretization effect on the friction wrench error}
%
%	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\hline
%		
%		\multirow{3}{*}{ID}	 & \multicolumn{12}{c|}{Wrench error with different sizes of elements (\%)} \\\cline{2-13}
%		
%		 & \multicolumn{2}{c|}{0.8} & \multicolumn{2}{c|}{0.7} & \multicolumn{2}{c|}{0.5} & \multicolumn{2}{c|}{0.3} & \multicolumn{2}{c|}{0.1}& \multicolumn{2}{c|}{0.01}\\ \cline{2-13}
%			 & U & H & U & H & U & H & U & H & U & H & U & H   \\ 
%		\hline
%		S1 & 8.1 &  & 6.5 &  & 3.8 & & 1.2 &   & 0.1 & && \\ \hline
%
%		
%		S2 & 10.7 &  & 10.7 &  & 5.6 & & 1.80 &  &  0.1 & && \\ \hline
%
%		S3 & 1.1 &  & 0.0 &  & 0.00 && 0.04 & & 0.0 &&& \\ \hline
%
%		
%		S4 & 1.1 &  & 0.0 &  & 0.00 && 0.04 & & 0.0 & &&\\ \hline
%
%		
%		S5 & 1.1 &  & 0.0 &  & 0.00 && 0.04 & & 0.0 & &&\\ \hline
%
%		
%		S6 & 1.1 &  & 0.0 &  & 0.00 && 0.04 & & 0.0 & 0.0 &&\\ \hline
%
%		\hline
%	\end{tabular}
%	\end{center}
%\end{table}



%\begin{table}
%	\begin{tabular}{|c|c|c|c|c|c|c|c|}
%		\hline
%		
%		ID	&\makecell{Pressure \\ distribution} & 0.8 & 0.7 & 0.5 & 0.4 & 0.3 & 0.1\\ 
%		\hline
%		\multirow{2}{*}{S1} & uniform & 0.0425 & 0.0342 & 0.0205 & 0.0108 & 0.0074 & 0.003\\
%		& Hertzian   & 0.0283 & 0.0207 & 0.0125 & 0.0069 & 0.0043 & 0.0017 \\ \hline
%		
%		\multirow{2}{*}{S2} & uniform &2.1 &2.1 & 2.1 & 2.1 & 2.1& \\ 
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6 & \\ \hline
%		
%		\multirow{2}{*}{S3} & uniform &2.1&2.1 & 2.1 & 2.1 & 2.1 &\\ 
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6 & \\ \hline
%		
%		\multirow{2}{*}{S4} & uniform &2.1 &2.1 & 2.1 & 2.1 & 2.1 &\\ 
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6 & \\	\hline	
%		
%		\multirow{2}{*}{S5} & uniform &2.1&2.1 & 2.1 & 2.1 & 2.1 &\\ 
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6& \\	\hline
%		
%		\multirow{2}{*}{S6} & uniform & 2.1 &2.1 & 2.1 & 2.1 & 2.1& \\ %\cmidrule{2-7}
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6 & \\ 	
%		\hline
%	\end{tabular}
%\end{table}



%\begin{table}
%	\begin{tabular}{|c|c|c|c|c|c|c|c|}
%		\hline
%		
%	ID	&\makecell{Pressure \\ distribution} & 0.8 & 0.7 & 0.5 & 0.4 & 0.3 & 0.1\\ 
%		\hline
%		\multirow{2}{*}{S1} & uniform & 0.0425 & 0.0342 & 0.0205 & 0.0108 & 0.0074 & 0.003\\
%		& Hertzian   & 0.0283 & 0.0207 & 0.0125 & 0.0069 & 0.0043 & 0.0017 \\ \hline
%
%		\multirow{2}{*}{S2} & uniform &2.1 &2.1 & 2.1 & 2.1 & 2.1& \\ 
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6 & \\ \hline
%		
%		\multirow{2}{*}{S3} & uniform &2.1&2.1 & 2.1 & 2.1 & 2.1 &\\ 
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6 & \\ \hline
%		
%		\multirow{2}{*}{S4} & uniform &2.1 &2.1 & 2.1 & 2.1 & 2.1 &\\ 
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6 & \\	\hline	
%		
%		\multirow{2}{*}{S5} & uniform &2.1&2.1 & 2.1 & 2.1 & 2.1 &\\ 
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6& \\	\hline
%		
%		\multirow{2}{*}{S6} & uniform & 2.1 &2.1 & 2.1 & 2.1 & 2.1& \\ %\cmidrule{2-7}
%		& Hertzian  & &11.6 & 11.6 & 11.6 & 11.6 & \\ 	
%		\hline
%	\end{tabular}
%\end{table}


==> tabs/tableLSParametricSurfaces.tex <==
\begin{table*}
	\begin{center}
		\caption{Fitting error of two limit surface models for the six parametric surfaces with three number of samples.}
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			\multirow{3}{*}{\makecell{Pressure \\ Distribution}}  & \multirow{3}{*}{ID} & \multicolumn{4}{c|}{Fitting error with 20 samples ($\%$)} & \multicolumn{4}{c|}{Fitting error with 150 samples ($\%$)} & \multicolumn{4}{c|}{Fitting error with 600 fitting samples ($\%$)}\\ \cline{3-14}
			
			& & \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Quadratic model}  & \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Quadratic model} & \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Quadratic model} \\ \cline{3-14}
			
			& & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist}  \\ 
			\hline
			
			\multirow{6}{*}{\makecell{Uniform \\ (U)}} & S1 & 13.67 & 37.04 & 11.50 & 36.47  &
			2.61 & 20.76 & 2.76 & 26.53  & 2.08 & 18.51 & 2.79 & 26.54  \\ \cline{2-14}
			
			& S2 & 13.98 & 33.04 & 5.65 & 31.55 & 2.39 & 17.00 & 2.94 & 24.78    & 1.88 & 15.07 & 3.07 & 23.53  \\  \cline{2-14}
			
			
			& S3  & 10.81 & 24.88 & 6.92 & 27.34 & 1.73 & 5.51 & 2.95 & 17.32  &  1.27 & 4.90 & 2.87 & 16.80  \\ \cline{2-14}
			
			
			& S4  & 8.74 & 21.51 & 4.33 & 21.41  & 1.64 & 5.65 & 3.04 & 16.49   & 1.17 & 4.76 & 3.17 & 16.51  \\ \cline{2-14}
			
			
			& S5  &13.34 & 44.93 & 3.85 & 28.50 & 2.85 & 18.69 & 2.66 & 25.78   &1.87 & 14.39 & 2.56 & 25.32  \\ \cline{2-14}
			
			
			& S6  & 9.13 & 34.34 & 4.80 & 31.31  &
			2.71 & 16.74 & 2.75 & 24.04  & 1.60 & 11.89 & 2.75 & 23.64  \\ %\cmidrule{2-7}
			\hline
			\hline
%			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\multirow{6}{*}{\makecell{Hetztian \\ (H)}} & S1  & 13.67 & 40.33 & 8.47 & 41.67 & 3.10 & 23.14 & 3.04 & 29.11  & 2.06 & 20.03 & 2.83 & 28.09 \\ \cline{2-14}
			
			& S2 & 11.25 & 30.33 & 6.69 & 36.29  & 
			2.76 & 17.59 & 2.65 & 24.38  & 1.99 & 15.63 & 3.06 & 24.13   \\ \cline{2-14}
			
			
			& S3  & 
			12.32 & 29.78 & 3.90 & 23.25 & 1.76 & 8.56 & 2.89 & 19.15 &1.19 & 8.30 & 2.76 & 18.87  \\ \cline{2-14}
			
			
			& S4 &9.03 & 21.56 & 5.45 & 23.59  & 1.62 & 6.30 & 2.95 & 17.43  & 1.18 & 5.57 & 3.02 & 17.46  \\ \cline{2-14}
			
			
			& S5 & 13.30 & 45.03 & 5.34 & 28.64  &
			2.79 & 19.08 & 2.59 & 26.04 & 1.85 & 14.63 & 2.64 & 25.32  \\ \cline{2-14}
			
			
			& S6 & 
			10.24 & 33.62 & 5.73 & 33.65 & 
			2.35 & 16.04 & 2.69 & 24.03 & 1.43 & 11.88 & 2.76 & 23.94  \\ %\cmidrule{2-7}
			\hline
			\hline
			\multicolumn{2}{|c|}{\textbf{Mean}} &
			 11.62 &  33.03  &  \textbf{6.05} &  \textbf{30.31}  &  \textbf{2.36}  & \textbf{14.59}  &  2.83  & 22.92  &  \textbf{1.63}  & \textbf{12.13} &   2.86 &  22.51  \\
			\hline
		\end{tabular}
	\end{center}
\end{table*}





%\begin{table*}
%	\begin{center}
%	\caption{Maximal integrated friction wrench and LS fitting results for the six parametric surfaces.}
%	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\hline
%		\multirow{3}{*}{P}  & \multirow{3}{*}{ID}  & \multirow{3}{*}{Maximal frictional force} & \multirow{3}{*}{Maximal frictional torque} & \multicolumn{4}{c|}{Fitting error with 100 samples ($\%$)} & \multicolumn{4}{c|}{Fitting error with 600 fitting samples ($\%$)}\\ \cline{5-12}
%		
%		 & & & & \multicolumn{2}{c|}{Quartic model} &
%		\multicolumn{2}{c|}{Quadratic model}  & \multicolumn{2}{c|}{Quartic model} &
%		\multicolumn{2}{c|}{Quadratic model}  \\ \cline{5-12}
%
%		& & & & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist}  \\ 
%		\cline{1-12}
%
%		\multirow{6}{*}{U} & S1 &  $[0.6366,0.6366,1.0000]^T$ & $[0.3405,0.6893,0.5947]^T$& 
%		5.62 & 25.33 & 3.35 & 32.00  & 2.08 & 18.51 & 2.79 & 26.54  \\ \cline{2-12}
%		
%		& S2 & $[0.8257,0.4129,1.0000]^T$  &$[0.1764,0.6429,0.3572]^T$ & 4.77 & 20.26 & 3.07 & 26.90   & 1.88 & 15.07 & 3.07 & 23.53  \\ \cline{2-12}
%		
%		
%		& S3 & $[0.7854,0.7854,0.7854]^T$ &$[0.5399,0.7854,0.5399]^T$ & 2.98 & 8.05 & 5.64 & 19.64   & 1.27 & 4.90 & 2.87 & 16.80  \\ \cline{2-12}
%
%		
%		& S4 & $[0.9074,0.6689,0.7617]^T$ &$[0.2881,0.5822,0.3862]^T$ & 2.07 & 6.77 & 3.95 & 16.99  & 1.17 & 4.76 & 3.17 & 16.51  \\ \cline{2-12}
%
%			
%		& S5 & $[0.8100,0.8100,0.7858]^T$ &$[0.2619,0.4613,0.4928]^T$& 4.93 & 24.74 & 3.19 & 26.83  & 1.87 & 14.39 & 2.56 & 25.32  \\ \cline{2-12}
%
%		
%		& S6 & $[0.8864,0.5905,0.8833]^T$ &$[0.1636,0.4741,0.3296^T$ & 3.41 & 20.46 & 3.55 & 25.44 & 1.60 & 11.89 & 2.75 & 23.64  \\ %\cmidrule{2-7}
%		\hline
%		\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		\multirow{6}{*}{H} & S1 &  $[0.6963,0.5837,1.0000]^T$ & $[0.3083,0.6451,0.5152]^T$& 5.86 & 28.70 & 3.22 & 33.50   & 2.06 & 20.03 & 2.83 & 28.09 \\ \cline{2-12}
%		
%		& S2 & $[0.8718,0.3515,1.0000]^T$  &$[0.1503,0.5936,0.2833]^T$ & 3.73 & 20.01 & 3.07 & 26.75 & 1.99 & 15.63 & 3.06 & 24.13   \\ \cline{2-12}
%		
%		
%		& S3 & $[0.8716,0.7273,0.8176]^T$ &$[0.4767,0.7274,0.4768]^T$ &3.60 & 10.68 & 4.13 & 21.14  & 1.19 & 8.30 & 2.76 & 18.87  \\ \cline{2-12}
%		
%		
%		& S4 & $[0.9357,0.6330,0.7619]^T$ &$[0.2805,0.5426,0.3338]^T$ & 2.65 & 8.35 & 3.92 & 18.05  & 1.18 & 5.57 & 3.02 & 17.46  \\ \cline{2-12}
%		
%		
%		& S5 & $[0.8303,0.7962,0.7809]^T$ &$[0.2440,0.4369,0.4591]^T$& 4.25 & 21.62 & 3.24 & 26.80 & 1.85 & 14.63 & 2.64 & 25.32  \\ \cline{2-12}
%		
%		
%		& S6 & $[0.9042,0.5658,0.8849]^T$ &$[0.1482,0.4491,0.2949]^T$ & 3.08 & 18.34 & 3.28 & 24.30  &  1.43 & 11.88 & 2.76 & 23.94  \\ %\cmidrule{2-7}
%		\hline
%	\end{tabular}
%	\end{center}
%\end{table*}
%


==> tabs/tableLSParametricSurfaces4cols.tex <==
\begin{table*}
	\begin{center}
		\caption{Fitting error of two limit surface models for the six parametric surfaces with three number of samples.}
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			\multirow{3}{*}{\makecell{Pressure \\ Distribution}}  & \multirow{3}{*}{ID} & \multicolumn{4}{c|}{Fitting error with 20 samples ($\%$)} & \multicolumn{4}{c|}{Fitting error with 150 samples ($\%$)} & \multicolumn{4}{c|}{Fitting error with 600 fitting samples ($\%$)}\\ \cline{3-14}
			
			& & \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Quadratic model}  & \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Quadratic model} & \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Quadratic model} \\ \cline{3-14}
			
			& & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist}  \\ 
			\hline
			
			\multirow{6}{*}{\makecell{Uniform \\ (U)}} & S1 & 13.67 & 37.04 & 11.50 & 36.47  &
			2.61 & 20.76 & 2.76 & 26.53  & 2.08 & 18.51 & 2.79 & 26.54  \\ \cline{2-14}
			
			& S2 & 13.98 & 33.04 & 5.65 & 31.55 & 2.39 & 17.00 & 2.94 & 24.78    & 1.88 & 15.07 & 3.07 & 23.53  \\  \cline{2-14}
			
			
			& S3  & 10.81 & 24.88 & 6.92 & 27.34 & 1.73 & 5.51 & 2.95 & 17.32  &  1.27 & 4.90 & 2.87 & 16.80  \\ \cline{2-14}
			
			
			& S4  & 8.74 & 21.51 & 4.33 & 21.41  & 1.64 & 5.65 & 3.04 & 16.49   & 1.17 & 4.76 & 3.17 & 16.51  \\ \cline{2-14}
			
			
			& S5  &13.34 & 44.93 & 3.85 & 28.50 & 2.85 & 18.69 & 2.66 & 25.78   &1.87 & 14.39 & 2.56 & 25.32  \\ \cline{2-14}
			
			
			& S6  & 9.13 & 34.34 & 4.80 & 31.31  &
			2.71 & 16.74 & 2.75 & 24.04  & 1.60 & 11.89 & 2.75 & 23.64  \\ %\cmidrule{2-7}
			\hline
			\hline
%			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\multirow{6}{*}{\makecell{Hetztian \\ (H)}} & S1  & 13.67 & 40.33 & 8.47 & 41.67 & 3.10 & 23.14 & 3.04 & 29.11  & 2.06 & 20.03 & 2.83 & 28.09 \\ \cline{2-14}
			
			& S2 & 11.25 & 30.33 & 6.69 & 36.29  & 
			2.76 & 17.59 & 2.65 & 24.38  & 1.99 & 15.63 & 3.06 & 24.13   \\ \cline{2-14}
			
			
			& S3  & 
			12.32 & 29.78 & 3.90 & 23.25 & 1.76 & 8.56 & 2.89 & 19.15 &1.19 & 8.30 & 2.76 & 18.87  \\ \cline{2-14}
			
			
			& S4 &9.03 & 21.56 & 5.45 & 23.59  & 1.62 & 6.30 & 2.95 & 17.43  & 1.18 & 5.57 & 3.02 & 17.46  \\ \cline{2-14}
			
			
			& S5 & 13.30 & 45.03 & 5.34 & 28.64  &
			2.79 & 19.08 & 2.59 & 26.04 & 1.85 & 14.63 & 2.64 & 25.32  \\ \cline{2-14}
			
			
			& S6 & 
			10.24 & 33.62 & 5.73 & 33.65 & 
			2.35 & 16.04 & 2.69 & 24.03 & 1.43 & 11.88 & 2.76 & 23.94  \\ %\cmidrule{2-7}
			\hline
			\hline
			\multicolumn{2}{|c|}{\textbf{Mean}} &
			 11.62 &  33.03  &  \textbf{6.05} &  \textbf{30.31}  &  \textbf{2.36}  & \textbf{14.59}  &  2.83  & 22.92  &  \textbf{1.63}  & \textbf{12.13} &   2.86 &  22.51  \\
			\hline
		\end{tabular}
	\end{center}
\end{table*}





%\begin{table*}
%	\begin{center}
%	\caption{Maximal integrated friction wrench and LS fitting results for the six parametric surfaces.}
%	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\hline
%		\multirow{3}{*}{P}  & \multirow{3}{*}{ID}  & \multirow{3}{*}{Maximal frictional force} & \multirow{3}{*}{Maximal frictional torque} & \multicolumn{4}{c|}{Fitting error with 100 samples ($\%$)} & \multicolumn{4}{c|}{Fitting error with 600 fitting samples ($\%$)}\\ \cline{5-12}
%		
%		 & & & & \multicolumn{2}{c|}{Quartic model} &
%		\multicolumn{2}{c|}{Quadratic model}  & \multicolumn{2}{c|}{Quartic model} &
%		\multicolumn{2}{c|}{Quadratic model}  \\ \cline{5-12}
%
%		& & & & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist} & {Wrench} & {Twist}  \\ 
%		\cline{1-12}
%
%		\multirow{6}{*}{U} & S1 &  $[0.6366,0.6366,1.0000]^T$ & $[0.3405,0.6893,0.5947]^T$& 
%		5.62 & 25.33 & 3.35 & 32.00  & 2.08 & 18.51 & 2.79 & 26.54  \\ \cline{2-12}
%		
%		& S2 & $[0.8257,0.4129,1.0000]^T$  &$[0.1764,0.6429,0.3572]^T$ & 4.77 & 20.26 & 3.07 & 26.90   & 1.88 & 15.07 & 3.07 & 23.53  \\ \cline{2-12}
%		
%		
%		& S3 & $[0.7854,0.7854,0.7854]^T$ &$[0.5399,0.7854,0.5399]^T$ & 2.98 & 8.05 & 5.64 & 19.64   & 1.27 & 4.90 & 2.87 & 16.80  \\ \cline{2-12}
%
%		
%		& S4 & $[0.9074,0.6689,0.7617]^T$ &$[0.2881,0.5822,0.3862]^T$ & 2.07 & 6.77 & 3.95 & 16.99  & 1.17 & 4.76 & 3.17 & 16.51  \\ \cline{2-12}
%
%			
%		& S5 & $[0.8100,0.8100,0.7858]^T$ &$[0.2619,0.4613,0.4928]^T$& 4.93 & 24.74 & 3.19 & 26.83  & 1.87 & 14.39 & 2.56 & 25.32  \\ \cline{2-12}
%
%		
%		& S6 & $[0.8864,0.5905,0.8833]^T$ &$[0.1636,0.4741,0.3296^T$ & 3.41 & 20.46 & 3.55 & 25.44 & 1.60 & 11.89 & 2.75 & 23.64  \\ %\cmidrule{2-7}
%		\hline
%		\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		\multirow{6}{*}{H} & S1 &  $[0.6963,0.5837,1.0000]^T$ & $[0.3083,0.6451,0.5152]^T$& 5.86 & 28.70 & 3.22 & 33.50   & 2.06 & 20.03 & 2.83 & 28.09 \\ \cline{2-12}
%		
%		& S2 & $[0.8718,0.3515,1.0000]^T$  &$[0.1503,0.5936,0.2833]^T$ & 3.73 & 20.01 & 3.07 & 26.75 & 1.99 & 15.63 & 3.06 & 24.13   \\ \cline{2-12}
%		
%		
%		& S3 & $[0.8716,0.7273,0.8176]^T$ &$[0.4767,0.7274,0.4768]^T$ &3.60 & 10.68 & 4.13 & 21.14  & 1.19 & 8.30 & 2.76 & 18.87  \\ \cline{2-12}
%		
%		
%		& S4 & $[0.9357,0.6330,0.7619]^T$ &$[0.2805,0.5426,0.3338]^T$ & 2.65 & 8.35 & 3.92 & 18.05  & 1.18 & 5.57 & 3.02 & 17.46  \\ \cline{2-12}
%		
%		
%		& S5 & $[0.8303,0.7962,0.7809]^T$ &$[0.2440,0.4369,0.4591]^T$& 4.25 & 21.62 & 3.24 & 26.80 & 1.85 & 14.63 & 2.64 & 25.32  \\ \cline{2-12}
%		
%		
%		& S6 & $[0.9042,0.5658,0.8849]^T$ &$[0.1482,0.4491,0.2949]^T$ & 3.08 & 18.34 & 3.28 & 24.30  &  1.43 & 11.88 & 2.76 & 23.94  \\ %\cmidrule{2-7}
%		\hline
%	\end{tabular}
%	\end{center}
%\end{table*}
%


==> tabs/tableRoboResults.tex <==
\begin{table}
	\begin{center}
		\caption{Prediction results with the quartic and ellipsoidal limit surface models.}
		\begin{tabular}{|c|c|c|c|c|c|}
			\hline
			\multirow{2}{*}{\makecell{Label \\ type}}  & \multirow{2}{*}{\makecell{Contact \\ type}}  	& \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Ellipsoidal model} \\ \cline{3-6}
			& & precision  & recall & precision & recall \\ \hline
			\multirow{3}{*}{\makecell{Camera}} & 1 &	0.986 & 0.636 & 0.985 & 0.626 \\ \cline{2-6}
			& 2 & 1.000 & 0.306 & 1.000 & 0.347 \\ \cline{2-6}
			& All & \textbf{0.991} & 0.461 & \textbf{0.991} & \textbf{0.478} \\ \hline
			\hline
			\multirow{3}{*}{Human} & 1 &	0.971 & 0.691 & 0.971 & 0.680 \\ \cline{2-6}
			& 2 &	0.973 & 0.419 & 0.929 & 0.453 \\ \cline{2-6}
			& All &\textbf{0.972} & 0.563 & 0.955 & \textbf{0.574} \\ \hline
%			\hline
%			\multirow{3}{*}{\makecell{Identical}} & 1 &	1.000 & 0.759 & 1.000 & 0.747 \\ \cline{2-6}
%			& 2 & 1.000 & 0.419 & 1.000 & 0.454\\ \cline{2-6}
%			& All &	\textbf{0.972} & 0.563 & 0.955 & \textbf{0.574} \\ \cline{2-6}						
%			\hline
		\end{tabular}
		\label{tab:expResults}
	\end{center}
\end{table}


%\begin{table}
%	\begin{center}
%		\caption{Prediction results with the quartic and ellipsoidal limit surface models.}
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			 \multirow{2}{*}{\makecell{Contact \\ type}}  	& \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Ellipsoidal model} \\ \cline{2-5}
%			 & precision  & recall & precision & recall \\ \hline
%			 1 &	0.972 & 0.722 & 0.972 & 0.722 \\ \hline
%			 2 &	0.976 & 0.465 & 0.930 & 0.465 \\ \hline
%			 All &	\textbf{0.973} & \textbf{0.601} & 0.957 & \textbf{0.601} \\ 		
%			\hline
%		\end{tabular}
%		\label{tab:expResults}
%	\end{center}
%\end{table}


%\begin{table}
%	\begin{center}
%		\caption{Prediction results with the quartic and ellipsoidal limit surface models.}
%		\begin{tabular}{|c|c|c|c|c|c|}
%			\hline
%			\multirow{2}{*}{\makecell{Samples \\ type}}  & \multirow{2}{*}{\makecell{Contact \\ type}}  	& \multicolumn{2}{c|}{Quartic model} & \multicolumn{2}{c|}{Ellipsoidal model} \\ \cline{3-6}
%			  & & precision  & recall & precision & recall \\ \hline
%			\multirow{3}{*}{All} & 1 &	0.972 & 0.722 & 0.972 & 0.722 \\ \cline{2-6}
%			& 2 &	0.976 & 0.465 & 0.930 & 0.465 \\ \cline{2-6}
%			& All &	\textbf{0.973} & \textbf{0.601} & 0.957 & \textbf{0.601} \\ \hline
%			\multirow{3}{*}{\makecell{Samples with \\ absolute  ground \\ truth  labels}} & 1 &	1.000 & 0.782 & 1.000 & 0.793 \\ \cline{2-6}
%			& 2 & 1.000 & 0.465 & 1.000 & 0.465\\ \cline{2-6}
%			& All &	\textbf{1.000} & 0.624 & \textbf{1.000} & \textbf{0.630} \\ \cline{2-6}						
%			\hline
%		\end{tabular}
%		\label{tab:expResults}
%	\end{center}
%\end{table}


%\begin{table*}
%	\begin{center}
%		\caption{Prediction results with the ellipsoidal and quartic polynomial limit surface models with a uniform and a Hertzian pressure distribution.}
%		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
%			\hline
%			\multirow{3}{*}{Type of samples}  & \multirow{3}{*}{Type of objects} & \multicolumn{4}{c|}{Prediction accuracy with initial normal forces (\%) } & \multicolumn{4}{c|}{Prediction accuracy with updated normal forces (\%) } \\ \cline{3-10}
%			
%			& & \multicolumn{2}{c|}{Quartic  LS model} & \multicolumn{2}{c|}{Elliptic LS  model} &  \multicolumn{2}{c|}{Quartic LS model} & \multicolumn{2}{c|}{Elliptic LS  model}\\ \cline{3-10}
%			&   & \makecell{Uniform} & \makecell{Hertzian} & \makecell{Uniform} & \makecell{Hertzian} & \makecell{Uniform} & \makecell{Hertzian} & \makecell{Uniform} & \makecell{Hertzian}  \\  \hline
%			\multirow{4}{*}{\makecell{All \\ samples} }  & 1  & 82.0& 79.0&88.0 &89.0 &87.0 &86.0 &90.0 &91.0 \\ \cline{2-10}
%			& 2  &80.0 &80.0 &76.7 &78.3 &75.0 &75.0 &75.0 &75.0\\  \cline{2-10}
%			& 3  & 67.5& 67.5&67.5 &67.5 &70.0 &70.0 &65.0 &65.0\\ \cline{2-10}
%			& \textbf{All }&78.5 &77.0 &80.5 &\textbf{81.5} &80.0 &79.5 &80.5 &\textbf{81.0}\\ \cline{2-10}
%			\hline
%			\hline
%			\multirow{4}{*}{\makecell{Samples with absolute \\   ground truth labels} }  & 1  & 81.1&78.4 &90.5 &91.9 &93.2 &89.2 &97.3 &98.6\\ \cline{2-10}
%			& 2 & 86.5& 86.5&83.8 &83.8 & 89.2&89.2 & 89.2&89.2\\  \cline{2-10}
%			& 3  &75.0 &75.0 &75.0 &75.0 &87.5 &87.5 &79.2 &79.2\\ \cline{2-10}
%			& \textbf{All}  & 81.5&80.0 &85.9 &\textbf{86.7} &91.1 &88.9 &91.9 &\textbf{92.6}\\ \cline{2-10}
%			\hline
%		\end{tabular}
%		\label{tab:expResults}
%	\end{center}
%\end{table*}

